A Symbolic Transformation Language and its Application to a Multiscale Method

The context of this work is the design of a software, called MEMSALab, dedicated to the automatic derivation of multiscale models of arrays of micro- and nanosystems. In this domain a model is a partial differential equation. Multiscale methods approximate it by another partial differential equation which can be numerically simulated in a reasonable time. The challenge consists in taking into account a wide range of geometries combining thin and periodic structures with the possibility of multiple nested scales. In this paper we present a transformation language that will make the development of MEMSALab more feasible. It is proposed as a Maple package for rule-based programming, rewriting strategies and their combination with standard Maple code. We illustrate the practical interest of this language by using it to encode two examples of multiscale derivations, namely the two-scale limit of the derivative operator and the two-scale model of the stationary heat equation.

==> GradientProof/gradient-output.tex <==
------ Reduction Of Left Hand Side Term--------
------ STEP 1 --------
 Integral({Y, TSTM(Omega)},T(gradient(u,x))*v,{x, y})
=
 Integral(Omega,TS(v)*gradient(u,x),{x})
----- STEP 2 ---------
=
 Integral(Omega,(bar(v)+BigO(1,Epsilon))*gradient(u,x),set(x))
=
 Integral(Omega,gradient(u,x)*bar(v)+gradient(u,x)*BigO(1,Epsilon),set(x))
=
 Integral(Omega,gradient(u,x)*bar(v),set(x))+Integral(Omega,gradient(u,x)*BigO(1,Epsilon),set(x))
=
 Integral(Omega,gradient(u,x)*bar(v),set(x))+BigO(5,Epsilon)
------- STEP 3 -------
=
 Integral({gradient(Omega)},u*bar(v)*Eta(x),{x})-Integral({Omega},u*div(bar(v),{x}),{x})+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*div(bar(v),set(x)),set(x))+BigO(5,Epsilon)
----- LHSTERM 4 ---------
=
 -Integral(set(Omega),u*(bar(div(v,set(x)))+1/Epsilon*bar(div(v,{y}))),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*bar(div(v,set(x)))+u/Epsilon*bar(div(v,{y})),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*bar(div(v,set(x))),set(x))-Integral(set(Omega),u/Epsilon*bar(div(v,{y})),set(x))+BigO(5,Epsilon)
----- LHSTERM 5 ---------
=
 -Integral(set(Omega),u*(TS(div(v,{x}))+BigO(3,Epsilon)),set(x))-Integral(set(Omega),u/Epsilon*bar(div(v,set(y))),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*(TS(div(v,set(x)))+BigO(3,Epsilon)),set(x))-Integral(set(Omega),u/Epsilon*(TS(div(v,{y})+Epsilon*y*partial(div(v,{y}),x))+Epsilon*BigO(4,Epsilon)),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x)))+u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u/Epsilon*TS(div(v,{y})+Epsilon*y*partial(div(v,{y}),x))+u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x)))+u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*(div(v,{y})+Epsilon*y*partial(div(v,{y}),x)))+u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x)))+u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*div(v,{y})+y*partial(div(v,{y}),x))+u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x))),set(x))-Integral(set(Omega),u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*div(v,{y})+y*partial(div(v,{y}),x)),set(x))-Integral(set(Omega),u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon) 
=
 -Integral(set(Omega),u*TS(div(v,set(x))),set(x))-Integral(set(Omega),u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x)),set(x))-Integral(set(Omega),u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon) 
=
 -Integral(set(Omega),u*TS(div(v,set(x))),set(x))-BigO(5,Epsilon)-Integral(set(Omega),u*TS(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x)),set(x))
----- LHSTERM 6 ---------
=
 -Integral({Y, TSTM(set(Omega))},div(v,set(x))*T(u),{x, y})-BigO(5,Epsilon)-Integral({Y, TSTM(set(Omega))},(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x))*T(u),{x, y})
------ LHSTERM 7 --------
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*(u({0})+BigO(9,Epsilon)),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x))*T(u),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*(u(set(0))+BigO(9,Epsilon)),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x))*(u({0})+Epsilon*tilde(u({1}))+Epsilon*BigO(10,Epsilon)),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0))+div(v,set(x))*BigO(9,Epsilon),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u({0})+div(v,set(y))*tilde(u({1}))+div(v,set(y))*BigO(10,Epsilon)+y*partial(div(v,set(y)),x)*u({0})+y*partial(div(v,set(y)),x)*Epsilon*tilde(u({1}))+y*partial(div(v,set(y)),x)*Epsilon*BigO(10,Epsilon),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*BigO(9,Epsilon),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*BigO(10,Epsilon),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*Epsilon*BigO(10,Epsilon),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*Epsilon*tilde(u(set(1))),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*BigO(9,Epsilon),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*BigO(10,Epsilon),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))-2*Integral(set(Y,TSTM(set(Omega))),7*BigO(8,Epsilon),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))-5*BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))+BigO(6,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))+BigO(6,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y)) 
------ LHSTERM 8  --------
=
 -Integral({partial(set(Y,TSTM(set(Omega))))},v*u(set(0))*Eta(set(x)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)-Integral({partial(set(Y,TSTM(set(Omega))))},v*tilde(u(set(1)))*Eta(set(y)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y)) 
=
 -Integral(set(partial(set(Y,TSTM(set(Omega))))),v*u(set(0))*Eta(set(x)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)-Integral(set(partial(set(Y,TSTM(set(Omega))))),v*tilde(u(set(1)))*Eta(set(y)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))-Integral({partial(set(Y,TSTM(set(Omega))))},div(v,set(y))*y*u(set(0))*Eta(x),set(x,y))+Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*div(y*u(set(0)),x),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*div(y*u(set(0)),x),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))+Integral({partial(set(Y,TSTM(set(Omega))))},v*div(y*u(set(0)),x)*Eta(set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(div(y*u(set(0)),x),set(y)),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(div(y*u(set(0)),x),set(y)),set(x,y)) 
------ LHSTERM 9  --------
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u({1})+y*div(u({0}),x),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(div(y*u(set(0)),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(1))+y*div(u(set(0)),x),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u({0}),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(1))+y*div(u(set(0)),x),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u({0}),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*(div(y*div(u(set(0)),x),set(y))+div(u(set(1)),set(y))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u(set(0)),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u(set(0)),x),set(y))+v*div(u(set(1)),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u(set(0)),x),set(y)),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(1)),set(y)),set(x,y)) 
------ Reduction Of Right Hand Side Term--------
=
 Integral({Y, TSTM(set(Omega))},v*div(u({0}),{x})+v*div(u({1}),{y}),{x, y})+BigO(11,Epsilon) 
=
 Integral({Y, TSTM(set(Omega))},v*div(u({0}),{x}),{x, y})+Integral({Y, TSTM(set(Omega))},v*div(u({1}),{y}),{x, y})+BigO(11,Epsilon) 
------------------------------ 
------  The  Left and Right Hand Side Terms matches up to:
=
 BigO(6,Epsilon) 


==> GradientProof/log.tex <==
                                                                                 23

                                             LHSterm := Integral({Y, TSTM(Omega)}, T(gradient(u(x), x)) v(x, y), {x, y})

                                                   LHSterm := Integral(Omega, TS(v(x, y)) gradient(u(x), x), {x})

                                                                                 23

                                       LHSterm := Integral(Omega, plus(bar(v(x, y)), BigO(Epsilon)) gradient(u(x), x), set(x))

                              LHSterm := Integral(Omega, plus(gradient(u(x), x) bar(v(x, y)), gradient(u(x), x) BigO(Epsilon)), set(x))

                 LHSterm := plus(Integral(Omega, gradient(u(x), x) bar(v(x, y)), set(x)), Integral(Omega, gradient(u(x), x) BigO(Epsilon), set(x)))

                                       LHSterm := plus(Integral(Omega, gradient(u(x), x) bar(v(x, y)), set(x)), BigO(Epsilon))

                                        step2 := plus(Integral(Omega, gradient(u(x), x) bar(v(x, y)), set(x)), BigO(Epsilon))

                                                                                 23

           step31 := plus(Integral({gradient(Omega)}, u(x) bar(v(x, y)) Eta(x), {x}) - Integral({Omega}, u(x) div(bar(v(x, y)), {x}), {x}), BigO(Epsilon))

                                     step3 := plus(-Integral(set(Omega), u(x) div(bar(v(x, y)), set(x)), set(x)), BigO(Epsilon))

                                                                                 23

                                                                 /                            bar(div(v(x, y), {y}))\
                       step41 := plus(-Integral(set(Omega), u(x) |bar(div(v(x, y), set(x))) + ----------------------|, set(x)), BigO(Epsilon))
                                                                 \                                   Epsilon        /

                                                                                           u(x) bar(div(v(x, y), {y}))
                     step42 := plus(-Integral(set(Omega), u(x) bar(div(v(x, y), set(x))) + ---------------------------, set(x)), BigO(Epsilon))
                                                                                                     Epsilon

                                                                                                          u(x) bar(div(v(x, y), {y}))
       step4 := plus(-Integral(set(Omega), u(x) bar(div(v(x, y), set(x))), set(x)) - Integral(set(Omega), ---------------------------, set(x)), BigO(Epsilon))
                                                                                                                    Epsilon

                                                                                 23

                                                                 subterm1 := bar(div(v(x, y), {x}))

                                                                                                                     u(x) bar(div(v(x, y), set(y)))
step51 := plus(-Integral(set(Omega), u(x) plus(TS(div(v(x, y), {x})), BigO(Epsilon)), set(x)) - Integral(set(Omega), ------------------------------, set(x)),
                                                                                                                                Epsilon

    BigO(Epsilon))

                                                                                                                           u(x) bar(div(v(x, y), set(y)))
step511 := plus(-Integral(set(Omega), plus(u(x) TS(div(v(x, y), {x})), u(x) BigO(Epsilon)), set(x)) - Integral(set(Omega), ------------------------------, set(x)),
                                                                                                                                      Epsilon

    BigO(Epsilon))

step512 := plus(-plus(Integral(set(Omega), u(x) TS(div(v(x, y), {x})), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x)))

                            u(x) bar(div(v(x, y), set(y)))
     - Integral(set(Omega), ------------------------------, set(x)), BigO(Epsilon))
                                       Epsilon

                                                                 subterm2 := bar(div(v(x, y), {y}))

step52 := plus(-plus(Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x)))

                            u(x) plus(TS(div(v(x, y), {y}) + Epsilon y partial(div(v(x, y), {y}), x)), Epsilon BigO(Epsilon))
     - Integral(set(Omega), -------------------------------------------------------------------------------------------------, set(x)), BigO(Epsilon))
                                                                         Epsilon

step53 := plus(-plus(Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x)))

                                 u(x) TS(div(v(x, y), {y}) + Epsilon y partial(div(v(x, y), {y}), x))
     - Integral(set(Omega), plus(--------------------------------------------------------------------, u(x) BigO(Epsilon)), set(x)), BigO(Epsilon))
                                                               Epsilon

step54 := plus(-plus(Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x)))

                                 u(x) TS(div(v(x, y), {y}) + Epsilon y partial(div(v(x, y), {y}), x))
     - plus(Integral(set(Omega), --------------------------------------------------------------------, set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x))),
                                                               Epsilon

    BigO(Epsilon))

step55 := plus(-plus(Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x)))

                                         div(v(x, y), {y}) + Epsilon y partial(div(v(x, y), {y}), x)
     - plus(Integral(set(Omega), u(x) TS(-----------------------------------------------------------), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x))),
                                                                   Epsilon

    BigO(Epsilon))

step56 := plus(-plus(Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x)))

                                         div(v(x, y), {y})
     - plus(Integral(set(Omega), u(x) TS(----------------- + y partial(div(v(x, y), {y}), x)), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x))),
                                              Epsilon

    BigO(Epsilon))

step57 := plus(plus(-Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x)))

                                          div(v(x, y), {y})
     + plus(-Integral(set(Omega), u(x) TS(----------------- + y partial(div(v(x, y), {y}), x)), set(x)), Integral(set(Omega), u(x) BigO(Epsilon), set(x))),
                                               Epsilon

    BigO(Epsilon))

step58 := plus(plus(

                                  div(v(x, y), {y})
    -Integral(set(Omega), u(x) TS(----------------- + y partial(div(v(x, y), {y}), x)), set(x)) - Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)),
                                       Epsilon

    2 Integral(set(Omega), u(x) BigO(Epsilon), set(x))), BigO(Epsilon))

memory used=38.4MB, alloc=37.4MB, time=0.18
step59 := plus(plus(

                                  div(v(x, y), set(y))
    -Integral(set(Omega), u(x) TS(-------------------- + y partial(div(v(x, y), set(y)), x)), set(x)) - Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)),
                                        Epsilon

    2 BigO(Epsilon)), BigO(Epsilon))

step5 := plus(

                                  div(v(x, y), set(y))
    -Integral(set(Omega), u(x) TS(-------------------- + y partial(div(v(x, y), set(y)), x)), set(x)) - Integral(set(Omega), u(x) TS(div(v(x, y), set(x))), set(x)),
                                        Epsilon

    3 BigO(Epsilon))

                                               /div(v(x, y), set(y))                                     \
step6 := plus(-Integral({Y, TSTM(set(Omega))}, |-------------------- + y partial(div(v(x, y), set(y)), x)| T(u(x)), {x, y})
                                               \      Epsilon                                            /

     - Integral({Y, TSTM(set(Omega))}, div(v(x, y), set(x)) T(u(x)), {x, y}), 3 BigO(Epsilon))

                                                   /div(v(x, y), set(y))                                     \
step71 := plus(-Integral(set(Y, TSTM(set(Omega))), |-------------------- + y partial(div(v(x, y), set(y)), x)| T(u(x)), set(x, y))
                                                   \      Epsilon                                            /

     - Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(x)) plus(u(x, {0}), BigO(Epsilon)), set(x, y)), 3 BigO(Epsilon))

step72 := plus(-Integral(set(Y, TSTM(set(Omega))),

    /div(v(x, y), set(y))                                     \
    |-------------------- + y partial(div(v(x, y), set(y)), x)| plus(u(x, {0}) + Epsilon tilde(u(x, {1})), Epsilon BigO(Epsilon)), set(x, y))
    \      Epsilon                                            /

     - Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(x)) plus(u(x, set(0)), BigO(Epsilon)), set(x, y)), 3 BigO(Epsilon))

                                                        /div(v(x, y), set(y))                                     \
step73 := plus(-Integral(set(Y, TSTM(set(Omega))), plus(|-------------------- + y partial(div(v(x, y), set(y)), x)| (u(x, {0}) + Epsilon tilde(u(x, {1}))),
                                                        \      Epsilon                                            /

    /div(v(x, y), set(y))                                     \
    |-------------------- + y partial(div(v(x, y), set(y)), x)| Epsilon BigO(Epsilon)), set(x, y))
    \      Epsilon                                            /

     - Integral(set(Y, TSTM(set(Omega))), plus(div(v(x, y), set(x)) u(x, set(0)), div(v(x, y), set(x)) BigO(Epsilon)), set(x, y)), 3 BigO(Epsilon))

                                  /div(v(x, y), set(y))                                     \
step74 := plus(-plus(Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| (u(x, {0}) + Epsilon tilde(u(x, {1}))), set(x, y)),
                                  \      Epsilon                                            /

                 /div(v(x, y), set(y))                                     \
    Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| Epsilon BigO(Epsilon), set(x, y)))
                 \      Epsilon                                            /

     - plus(Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y)), Integral(%1, div(v(x, y), set(x)) BigO(Epsilon), set(x, y))), 3 BigO(Epsilon))

%1 := set(Y, TSTM(set(Omega)))

memory used=76.6MB, alloc=39.7MB, time=0.28
                                  /div(v(x, y), set(y))                                     \
step75 := plus(plus(-Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| (u(x, {0}) + Epsilon tilde(u(x, {1}))), set(x, y)),
                                  \      Epsilon                                            /

                 /div(v(x, y), set(y))                                     \
    Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| Epsilon BigO(Epsilon), set(x, y)))
                 \      Epsilon                                            /

     + plus(-Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y)), Integral(%1, div(v(x, y), set(x)) BigO(Epsilon), set(x, y))), 3 BigO(Epsilon))

%1 := set(Y, TSTM(set(Omega)))

                             /div(v(x, y), set(y))                                     \
step76 := plus(-Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| (u(x, {0}) + Epsilon tilde(u(x, {1}))), set(x, y))
                             \      Epsilon                                            /

     + plus(-Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y)), Integral(%1, div(v(x, y), set(x)) BigO(Epsilon), set(x, y))),

                                   /div(v(x, y), set(y))                                     \
    3 BigO(Epsilon) + Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| Epsilon BigO(Epsilon), set(x, y)))
                                   \      Epsilon                                            /

%1 := set(Y, TSTM(set(Omega)))

step77 := plus(-Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y))

                    /div(v(x, y), set(y))                                     \
     - Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| (u(x, {0}) + Epsilon tilde(u(x, {1}))), set(x, y)), 3 BigO(Epsilon)
                    \      Epsilon                                            /

                    /div(v(x, y), set(y))                                     \
     + Integral(%1, |-------------------- + y partial(div(v(x, y), set(y)), x)| Epsilon BigO(Epsilon), set(x, y))
                    \      Epsilon                                            /

     + Integral(%1, div(v(x, y), set(x)) BigO(Epsilon), set(x, y)))

%1 := set(Y, TSTM(set(Omega)))

                                                                                          div(v(x, y), set(y)) u(x, {0})
step78 := plus(-Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y)) - Integral(%1, ------------------------------ + div(v(x, y), set(y)) tilde(u(x, {1}))
                                                                                                     Epsilon

     + y partial(div(v(x, y), set(y)), x) u(x, {0}) + y partial(div(v(x, y), set(y)), x) Epsilon tilde(u(x, {1})), set(x, y)), 3 BigO(Epsilon)

     + Integral(%1, BigO(Epsilon) div(v(x, y), set(y)) + Epsilon BigO(Epsilon) y partial(div(v(x, y), set(y)), x), set(x, y))

     + Integral(%1, div(v(x, y), set(x)) BigO(Epsilon), set(x, y)))

%1 := set(Y, TSTM(set(Omega)))

step79 := plus(-Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(x)) u(x, set(0)), set(x, y)) - Integral(set(Y, TSTM(set(Omega))),

    div(v(x, y), set(y)) u(x, set(0))
    --------------------------------- + div(v(x, y), set(y)) tilde(u(x, set(1))) + y partial(div(v(x, y), set(y)), x) u(x, set(0))
                 Epsilon

     + y partial(div(v(x, y), set(y)), x) Epsilon tilde(u(x, set(1))), set(x, y)),

    4 BigO(Epsilon) + Integral(set(Y, TSTM(set(Omega))), BigO(Epsilon) div(v(x, y), set(y)) + Epsilon BigO(Epsilon) y partial(div(v(x, y), set(y)), x), set(x, y)))

step791 := plus(-Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y)) - Integral(%1, div(v(x, y), set(y)) tilde(u(x, set(1))), set(x, y)) - Integral(%1,

    div(v(x, y), set(y)) u(x, set(0))
    --------------------------------- + y partial(div(v(x, y), set(y)), x) u(x, set(0)) + y partial(div(v(x, y), set(y)), x) Epsilon tilde(u(x, set(1))), set(x, y))
                 Epsilon

    , 4 BigO(Epsilon) + Integral(%1, BigO(Epsilon) div(v(x, y), set(y)), set(x, y))

     + Integral(%1, Epsilon BigO(Epsilon) y partial(div(v(x, y), set(y)), x), set(x, y)))

%1 := set(Y, TSTM(set(Omega)))

memory used=114.9MB, alloc=39.7MB, time=0.38
step792 := plus(-Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(x)) u(x, set(0)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(y)) tilde(u(x, set(1))), set(x, y)) - Integral(set(Y, TSTM(set(Omega))),

    div(v(x, y), set(y)) u(x, set(0))
    --------------------------------- + y partial(div(v(x, y), set(y)), x) u(x, set(0)) + y partial(div(v(x, y), set(y)), x) Epsilon tilde(u(x, set(1))), set(x, y))
                 Epsilon

    , 6 BigO(Epsilon))

intern := plus(-Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(x)) u(x, set(0)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(y)) tilde(u(x, set(1))), set(x, y)) - Integral(set(Y, TSTM(set(Omega))),

    div(v(x, y), set(y)) u(x, set(0))
    --------------------------------- + y partial(div(v(x, y), set(y)), x) u(x, set(0)) + y partial(div(v(x, y), set(y)), x) Epsilon tilde(u(x, set(1))), set(x, y))
                 Epsilon

    , 6 BigO(Epsilon))

memory used=153.1MB, alloc=40.5MB, time=0.46
step793 := plus(-Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y)) - Integral(%1, div(v(x, y), set(y)) tilde(u(x, set(1))), set(x, y))

                                                                                               div(v(x, y), set(y)) u(x, set(0))
     - Integral(%1, y partial(div(v(x, y), set(y)), x) u(x, set(0)), set(x, y)) - Integral(%1, ---------------------------------, set(x, y))
                                                                                                            Epsilon

     - Integral(%1, y partial(div(v(x, y), set(y)), x) Epsilon tilde(u(x, set(1))), set(x, y)), 6 BigO(Epsilon))

%1 := set(Y, TSTM(set(Omega)))

memory used=191.2MB, alloc=41.8MB, time=0.52
step794 := plus(-Integral(%1, div(v(x, y), set(x)) u(x, set(0)), set(x, y)) - Integral(%1, div(v(x, y), set(y)) tilde(u(x, set(1))), set(x, y))

                                                                                               div(v(x, y), set(y)) u(x, set(0))
     - Integral(%1, y partial(div(v(x, y), set(y)), x) u(x, set(0)), set(x, y)) - Integral(%1, ---------------------------------, set(x, y)), 6 BigO(Epsilon))
                                                                                                            Epsilon

%1 := set(Y, TSTM(set(Omega)))

memory used=229.5MB, alloc=42.4MB, time=0.60
step7 := plus(-Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(x)) u(x, set(0)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(y)) tilde(u(x, set(1))), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), y partial(div(v(x, y), set(y)), x) u(x, set(0)), set(x, y)), 6 BigO(Epsilon))

step81 := plus(-Integral({partial(%1)}, v(x, y) u(x, set(0)) Eta(set(x)), set(x, y)) + Integral(%1, v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     - Integral({partial(%1)}, v(x, y) tilde(u(x, set(1))) Eta(set(y)), set(x, y)) + Integral(%1, v(x, y) div(tilde(u(x, set(1))), set(y)), set(x, y))

     - Integral(%1, y partial(div(v(x, y), set(y)), x) u(x, set(0)), set(x, y)), 6 BigO(Epsilon))

%1 := set(Y, TSTM(set(Omega)))

memory used=267.9MB, alloc=44.1MB, time=0.67
step82 := plus(-Integral(set(partial(%1)), v(x, y) u(x, set(0)) Eta(set(x)), set(x, y)) + Integral(%1, v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     - Integral(set(partial(%1)), v(x, y) tilde(u(x, set(1))) Eta(set(y)), set(x, y)) + Integral(%1, v(x, y) div(tilde(u(x, set(1))), set(y)), set(x, y))

     - Integral({partial(%1)}, div(v(x, y), set(y)) y u(x, set(0)) Eta(x), set(x, y)) + Integral(%1, div(v(x, y), set(y)) div(y u(x, set(0)), x), set(x, y)),

    6 BigO(Epsilon))

%1 := set(Y, TSTM(set(Omega)))

step83 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) div(tilde(u(x, set(1))), set(y)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), div(v(x, y), set(y)) div(y u(x, set(0)), x), set(x, y)), 6 BigO(Epsilon))

memory used=306.3MB, alloc=44.1MB, time=0.74
step84 := plus(Integral(%1, v(x, y) div(u(x, set(0)), set(x)), set(x, y)) + Integral(%1, v(x, y) div(tilde(u(x, set(1))), set(y)), set(x, y))

     + Integral({partial(%1)}, v(x, y) div(y u(x, set(0)), x) Eta(set(y)), set(x, y)) - Integral(%1, v(x, y) div(div(y u(x, set(0)), x), set(y)), set(x, y)),

    6 BigO(Epsilon))

%1 := set(Y, TSTM(set(Omega)))

step8 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) div(tilde(u(x, set(1))), set(y)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), v(x, y) div(div(y u(x, set(0)), x), set(y)), set(x, y)), 6 BigO(Epsilon))

step91 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, {1}) + y div(u(x, {0}), x), set(y)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), v(x, y) div(div(y u(x, set(0)), x), set(y)), set(x, y)), 6 BigO(Epsilon))

memory used=344.5MB, alloc=44.8MB, time=0.80
step92 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(1)) + y div(u(x, set(0)), x), set(y)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), v(x, y) div(y div(u(x, {0}), x), set(y)), set(x, y)), 6 BigO(Epsilon))

step93 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(1)) + y div(u(x, set(0)), x), set(y)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), v(x, y) div(y div(u(x, {0}), x), set(y)), set(x, y)), 6 BigO(Epsilon))

memory used=382.8MB, alloc=44.8MB, time=0.88
step94 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) (div(y div(u(x, set(0)), x), set(y)) + div(u(x, set(1)), set(y))), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), v(x, y) div(y div(u(x, set(0)), x), set(y)), set(x, y)), 6 BigO(Epsilon))

step95 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) div(y div(u(x, set(0)), x), set(y)) + v(x, y) div(u(x, set(1)), set(y)), set(x, y))

     - Integral(set(Y, TSTM(set(Omega))), v(x, y) div(y div(u(x, set(0)), x), set(y)), set(x, y)), 6 BigO(Epsilon))

step96 := plus(Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(0)), set(x)), set(x, y))

     + Integral(set(Y, TSTM(set(Omega))), v(x, y) div(u(x, set(1)), set(y)), set(x, y)), 6 BigO(Epsilon))

memory used=414.2MB, alloc=44.8MB, time=0.93


==> about.tex <==
Cette partie documente la rédaction d'un article refusé pour un numéro
spécial de JSC en 2011, mais accepté en 2013 dans la revue JSC.

Sections~\ref{about:jsc:abstract:sec} and the following sections give comments
about the corresponding parts in the paper.

\subsection{Comment évaluer les preuves ?}
Les fichiers de preuves dans le sous-dossier \url{GradientProof} sont des
variantes des fichiers de même nom, dans le dossier 

\url{/org/MEMSALab/software/memsalab/src/symbtrans/examples/}

distribué avec symbtrans. On ne peut pas évaluer les preuves ici. Il faut ce
placer dans le dossier 

\url{/org/MEMSALab/software/memsalab/src/symbtrans/examples/}

et suivre les instructions du fichier
\url{/org/MEMSALab/software/memsalab/src/symbtrans/readme.txt}.

\subsection{Résumé en français}
A conserver (pour hal) et à mettre à jour :

Le paradigme à deux échelles est une approche de dérivation de modèles pour les
matrices de microsystèmes. Ces modèles sont exprimés en terme d'équations
différentielles.

Il existe d'une part une correspondance naturelle entre les dérivations
mathématiques (c'est-à-dire le raisonnement équationnel) et la réécriture.
D'autre part, le langage de programmation Maple (utilisé par nos partenaires) a
peu de fonctionnalités de réécriture.

Nous fournissons un package Maple contenant des fonctions et des  stratégies de
réécriture. On applique ces fonctions pour donner une preuve semi-automatique
d'une propriété de convergence faible de l'action d'un opérateur de
transformation à deux échelles sur le gradient d'une fonction.

\subsection{TODO}

\subsubsection{For JSC}
Après acceptation, pour la version finale.

\begin{itemize}
\item ``owrds'' -``words'' [AG : Fait]

\item Example 10: dy au lieu de x ? [AG : Inutile, dans une partie supprimée]

\item AG : Révision des affiliations. [Fait]

\item WB : Réviser affiliation si nécessaire.

\item ML : Réviser adresse affiliation. [Fait]

\item Ajout support Labex ACTION et PPF Midi. [AG : Fait]

\item Revise the content of the included .mpl files. [AG : Fait]

\item Re-generate gradient-input.tex and heat-input.tex. [AG : Fait, à la main]

\item Suppression de toute la partie 3.5, sur le ``contextual rewriting''.
[AG : fait] La définition actuelle de la transformation \texttt{InnerContext}
dans l'article ne résout pas le problème pour lequel elle est introduite
(l'appliquer à la main pour le constater). De plus, cette transformation n'est
jamais utilisée dans le code Maple des preuves. Pour l'étape 8, qui correspond
au problème soulevé dans l'article, ce code utilise la règle conditionnelle
\texttt{CondGreenRule}, qui utilise la fonction Maple \texttt{has} pour détecter
un pattern.

La transformation \texttt{OuterContext} n'est utilisée que deux fois dans les
preuves Maple, dans les étapes 5 et 7 de la preuve du gradient. L'étape 5 sert
d'ailleurs d'exemple dans l'article.

Dans l'étape 5, on peut avantageusement se passer de la transformation
\texttt{OuterContext} en remplaçant
\begin{verbatim}
multContext := [X_,(1/Epsilon)*X*Y_];
ApproximationTSInv2Context :=
  OuterContext(ApproximationB[2](x(j))(y(j))(j))(multContext);
LHSterm := OutermostNF(ApproximationTSInv2Context)(LHSterm);
\end{verbatim}
par
\begin{verbatim}
ApproximationTSInv2Context :=
 Comp([
  [(1/Epsilon)*X_,(1/Epsilon)*X],
  Outermost(ApproximationB[2](x(j))(y(j))(j))
 ]);
LHSterm := OutermostNF(ApproximationTSInv2Context)(LHSterm);
\end{verbatim}
sachant que 
\begin{verbatim}
ApproximationB := [
  [B(V_), DelayEval -> TS(V)+BigO(FreshIndex(),Epsilon)],
  x -> y -> j -> [
     B(V_),
     TS(V+Epsilon*SUM(y*partial(V,x),j,J)) 
      + Epsilon*BigO(FreshIndex(),Epsilon)
  ]
];
\end{verbatim}

Ce changement remplace l'expression
\begin{verbatim}
LHSterm := -SUM(Integral(Omega, u B(partial(v(i), x(i))), x), i, Iset) - SUM(

    Integral(Omega, (TS(partial(v(i), y(i))

     + Epsilon SUM(y(j) partial(partial(v(i), y(i)), x(j)), j, J))

     + Epsilon BigO(5, Epsilon)) u/Epsilon, x), i, Iset) + BigO(4, Epsilon)
\end{verbatim}
par l'expression équivalente
\begin{verbatim}
LHSterm := -SUM(Integral(Omega, u B(partial(v(i), x(i))), x), i, Iset) - SUM(

    Integral(Omega, u (TS(partial(v(i), y(i))

     + Epsilon SUM(y(j) partial(partial(v(i), y(i)), x(j)), j, J))

     + Epsilon BigO(5, Epsilon))/Epsilon, x), i, Iset) + BigO(4, Epsilon)
\end{verbatim}
et mène au même résultat final. 

Dans l'étape 7, on peut remplacer
\begin{verbatim}
multContext := [X_,X*(1/Epsilon*Y_)];
ApproximationT2Context := OuterContext(ApproximationT[2])(multContext);
LHSterm := Outermost(ApproximationT2Context)(LHSterm);
\end{verbatim}
par
\begin{verbatim}
ApproximationT2Context :=
 Comp([
  [(1/Epsilon)*X_,(1/Epsilon)*X],
  Outermost(ApproximationT[2])
 ]);
LHSterm := Outermost(ApproximationT2Context)(LHSterm);
\end{verbatim}

Ce changement remplace l'expression
\begin{verbatim}
LHSterm := BigO(16, Epsilon) - SUM(

    Integral([TSTM(Omega), TSTm(Omega)], partial(v(i), x(i)) T(u), [x, y]), i,

    Iset) - SUM(Integral([TSTM(Omega), TSTm(Omega)], (u0 + Epsilon u1

     + Epsilon SUM(y(j) partial(u0, x(j)), j, J) + Epsilon BigO(17, Epsilon))

    partial(v(i), y(i))/Epsilon, [x, y]), i, Iset) - SUM(Integral(

    [TSTM(Omega), TSTm(Omega)],

    SUM(y(j) partial(partial(v(i), y(i)), x(j)), j, J) T(u), [x, y]), i, Iset)
\end{verbatim}
par l'expression équivalente
\begin{verbatim}
LHSterm := BigO(16, Epsilon) - SUM(

    Integral([TSTM(Omega), TSTm(Omega)], partial(v(i), x(i)) T(u), [x, y]), i,

    Iset) - SUM(Integral([TSTM(Omega), TSTm(Omega)], partial(v(i), y(i)) (u0

     + Epsilon u1 + Epsilon SUM(y(j) partial(u0, x(j)), j, J)

     + Epsilon BigO(17, Epsilon))/Epsilon, [x, y]), i, Iset) - SUM(Integral(

    [TSTM(Omega), TSTm(Omega)],

    SUM(y(j) partial(partial(v(i), y(i)), x(j)), j, J) T(u), [x, y]), i, Iset)
\end{verbatim}
et mène au même résultat final. 

Ceci est validé dans le fichier 
\url{/org/MEMSALab/software/memsalab/src/symbtrans/examples/gradient.mpl}
et fait dans les fichiers
\url{/org/MEMSALab/paper/JSCspecial11/GradientProof/gradient.mpl} et
\url{/org/MEMSALab/paper/JSCspecial11/GradientProof/gradient-input.tex}.

\item En ajoutant ``term'' dans la phrase ``In particular terms, patterns,
rules, strategies, pattern matching and application of rules and strategies to
terms are represented by Maple expressions.'', on dit que ``expression'' et
``term'' sont synonymes, pour pouvoir utiliser les deux indifféremment. Le
premier se rapporte plus à Maple, le second est plus général. [Fait]

\item Remplacement de \verb+A+ par \verb+_+, par exemple dans

\begin{verbatim}
    LinearityOf[Integral] := Linearity(2,x->y->x+y,Integral(Omega_,A,Z_));
\end{verbatim}
  dans integral.mpl, comme expliqué dans advanced.tex (section 5.2).
  De même dans twoscale.mpl. [Fait]

\item Pour éviter la confusion avec les constantes, ne parler que de
``scalaire'' pour la linéarité. [Fait]

\item Essai de déplacement de OutermostNF de stmodule.mpl vers gradient.mpl et
heat.mpl. Echec. Cause non identifiée. Abandon. [Fait]

\item La linéarité n'étant pas une transformation symbolique générale,
elle ne devrait pas être implantée dans symbtrans. Malheureusement, elle
l'est et dépend d'autres fonctions utiles de symbtrans, comme
UnderscoreElim. Il est donc difficile de l'enlever. On la conserve dans
symbtrans, mais en archivant ce commentaire pour re-considérer ce problème
ultérieurement. [Fait]
 
\item Remplacement de $s(t_i)$ par $\texttt{Transform}(s)(t_i)$ dans la
définition de \texttt{All} dans rhomaple.tex, conformément au code.
Voir test[31] dans regtest.mpl. [Fait]

\item Maple -> \textsf{Maple} ? [Ignoré]
 
\item Avant d'envoyer la version finale, regrouper tout le LaTeX dans un seul
fichier BGL.tex.

\item Eliminer les ``Overfull hbox'' de la compilation LaTeX.
\end{itemize}

\subsubsection{After JSC}
\begin{itemize}
\item Améliorer le texte au début de l'annexe A, en fonction de ce qui est écrit
dans la partie ``Formal proof examples''. Préciser au début de l'annexe A quelle
partie de la Proposition 3 est prouvée. Exprimer cette partie comme un lemme ?
Ajouter un environnement proof autour de cette preuve.

\item Explication annexe E : hypothesis vs. lemma : les lemmes sont généraux,
les hypothèses sont liées au modèle/problème particulier.

\item A propos de lemmas.mpl : dire que ce sont des règles qu'on
démontrera plus tard. On en démontre une : c'est l'approximation du gradient. 

\item Renommer le fichier integral.mpl, qui ne contient pas que des règles pour
les intégrales. [Facultatif]

\item Déplacer GradientApprox dans lemmas.mpl. [Facultatif]

\item Relier E.1 avec l'annexe A de [LS07]. [Facultatif]

\item Remplacer partout \texttt{Identity} par \texttt{Id}, plus court ?
[Facultatif]

\item A faire pour la preuve de l'équation de diffusion :

\begin{enumerate}
 \item Améliorer l'introduction de l'annexe B.
 \item Il manque des O(Epsilon) dans la preuve mathématique ?
 \item Expliquer les factorisations ad hoc ajoutées (factor1, factor2) at Step 2.
 (Il manque des règles de linéarité inverses pour effectuer ces regroupements).
\end{enumerate}

\item Améliorer : On trouve des exemples avec des intégrales d'arité 2 et
d'autres d'arité 3.

Enlever InnerContext/OuterContext dans symbtrans ?

\item Explain how ``The user can also extend the language with other
strategies.'' when symbtrans is provided as a Maple module.
 
\item TopDown et BottomUp ne sont pas bien expliqués. Ajouter un exemple, qui
montre que c'est différent de Outermost, Innermost et STNormalizer.

\item Comparer avec l'article d'Augustin ?  Gradient : reduction
séparée des deux membres. Diffusion : réduction simultanée des deux membres,
égalité codée par une différence. 

\item Remplacer l'hypothèse ``$u0$ ne dépend pas de $y$'' par une preuve séparée
de la règle U0IndependentOfY, avec la règle \verb+Integral(X_*v) = 0 -> X = 0+.

\item Ajouter cette remarque dans une version longue :
 Pour Maple, I est le nombre complexe dont le carré est -1.
  On évite donc d'utiliser I comme ensemble de sommation.
  On le remplace partout par Iset.

\item Expliquer qu'on peut enlever Transform, sauf ``for top rewriting''.

\item Faire une grammaire des stratégies :

\begin{align*}
strategy/transformation ::= 
  Transform(rule) \;|\; 
  Identity \;|\;
  Fail \;|\;
  IdentityAsFail(strategy) \;|\;
  FailAsIdentity(strategy) \;|\;
  All(strategy) \;|\;
  TopDown(strategy) \;|\;
  BottomUp(strategy) \;|\;
(t,\cdots,t)
\end{align*}

\item Remplacer les hypothèses dépendantes des données par des instantiations
de fonctions plus générales, comme dans le cas des ``Partial*0IndependentOfY''.

\item Pourquoi 

partialBound([Omega, x(i)])

dans la preuve formelle, et pas

partialBound([Omega])

comme dans la preuve mathématique ?

Devrait être partialBound([Omega, x]) ?

\item Développer une transformation des expressions Maple en formules LaTeX et
les appliquer aux fichiers de sortie de preuve. Voir partie~\ref{proof:pp:sec}.

\item Améliorer le step 6 de la preuve B.
\begin{verbatim}
# The result of the gradient proof is turned into the following
# rewrite rule. Formally, the symbols u, x, y, i, K and v(i) have been respectively
# replaced by the variables U_, X_, Y_, I_, K_, V_ [TODO: justify for v(i)]
# Bug with X_(I_) matching. 
GradientApprox := [
  SUM(
    Integral(
      [TSTM(Omega), TSTm(Omega)],
      T(partial(U_,X_(I_)))*V_,
      [X_, Y_]),
    I_,K_),
  DelayEval -> SUM(
    Integral(
      [TSTM(Omega), TSTm(Omega)],
      (partial(u0,X(I))+partial(u1,Y(I)))*V,
      [X, Y]),
    I,K)+BigO(FreshIndex(),Epsilon)];


  
# Here, we just check that it matches with the result of the 
# formal gradient proof. 
# read `gradient-output.mpl`:
# printf("%a\n = \n ", op(1,stepList[1]));
# printf("%a\n\n", op(1,stepList[2]));

\end{verbatim}
\begin{verbatim}
# TODO: replace by weak convergence coming from other files as follows
# after adaptation as in normal.mpl. 

# TODO : Maple version of gradient.prf.
read `gradient.prf`:
# We have proved that  
result1 := op(1,stepList[1]) = op(1,stepList[2]) + op(1,stepList[3]);
# thus that we can use result1 as a rewrite rule in diffusion_equation.mpl.
# TODO: replace GradientApproximation by result1.
# - Introduce variables (underscore) in op(1,stepList[1]).
# Replace this support by file by a support by procedures.
\end{verbatim}


\item Oter ce qui suit, si ce n'est pas utilisé : 
\begin{verbatim}
# 5. Hypotheses

VariablesOf[v] := {x,x(i)}:
VariablesOf[v0] := {x,x(i)}:
VariablesOf[v1] := {y(i),x,x(i)}:

# 6. Auxiliary functions
VariablesSetList := L -> 
  if (L = []) then 
    [];
  else
    [op(VariablesSet(L[1])), op(VariablesSetList(subsop(1=NULL,L)))];
  fi:

VariablesSet := t ->
  if member([t],{indices(VariablesOf)}) then
    VariablesOf[t];
  else
    if IsLeaf(t) then
      [];
    else
      VariablesSetList(ListParam(t));
    fi;
  fi:
\end{verbatim}

\item Find the bug when using this rule for step 6 of the diffusion equation
(\verb+matching X_(I_)+)

\begin{verbatim}
GradientApprox := [
  SUM(
    Integral(
      [TSTM(Omega), TSTm(Omega)],
      T(partial(U_,X_(I_)))*V_,
      [X_, Y_]),
    I_,K_),
  DelayEval -> SUM(
    Integral(
      [TSTM(Omega), TSTm(Omega)],
      (partial(u0,X(I))+partial(u1,Y(I)))*V,
      [X, Y]),
    I,K)+BigO(FreshIndex(),Epsilon)];
\end{verbatim}
\end{itemize}

\subsection{Code dissemination}
\label{symbtrans:dissemination:sec}
Un relecteur de JSC souhaite utiliser notre langage de stratégies. Nous devons
donc choisir un mode de distribution, qui doit satisfaire les exigences
suivantes :
\begin{enumerate}
\item Faible coût de maintenance du support de diffusion et de la version distribuée.
\item Identification des utilisateurs, pour envisager des collaborations.
\item Description d'un mode d'obtention pérenne dans l'article.
\end{enumerate}

La version de \texttt{symbtrans} présentée dans l'article sera distribuée sous
la forme d'une archive zip et/ou tar.gz.

On a choisi de diffuser uniquement auprès des relecteurs. C'est le minimum requis.
Le package peut être envoyé à l'éditeur en chef, avec un argument de
confidentialité :

Lu sur
\url{http://www.elsevier.com/wps/find/journaldescription.cws_home/622902/authorinstructions}:
``Supplementary Material: Please send the supplementary material, if any, to the
Editor-In-Chief, Professor Hoon Hong.''

Avantages :  Diffusion limitée.

Inconvénients : Peut être considéré comme insuffisant par un relecteur. Un
argument pourrait être : ``Dans son niveau d'avancement actuel, le package est
destiné à un usage au sein de projets de recherche auxquels ses auteurs
participent. Nous ne disposons pas encore d'assez de moyens humains pour
gérer les retours d'une large communauté.'' 

Une autre possibilité aurait été la  diffusion auprès des lecteurs de la
revue.
	
Inconvénients : Diffusion plus large, donc maintenance plus lourde (gestion de
rapports de bugs, \ldots). Nécessite une mention dans l'article, sur le mode
d'obtention du package. Si cette mention se veut aussi pérenne que l'article,
c'est à dire que la revue qui le diffuse, l'idéal serait que le package soit
aussi diffusé par la revue, mais cette possibilité n'existe pas, et pose des
problèmes de droits et de propriété intellectuelle. La pérennité de la diffusion
dépend de son support. Un site web ne satisfait pas les exigences ci-dessus, car
les adresses web changent sans que les auteurs le décident, ni même n'en soient
avertis (sauf site personnel d'un des auteurs, qui ne répond pas à l'exigence
1). 

Exemple de présentation de logiciel vu dans un article JSC :
Footnote: ``Venus is a free software; it can be downloaded at
http://rap.dsi.unifi.it/cows and can be redistributed the terms of the GNU
General Public License as published by the Free Software Foundation.''


\subsection{Submission to JSC in 2011}
Messages échangés, dans l'ordre chronologique inverse.

\subsubsection{Acceptation message}
Sujet: JSC YJSCO-7601. De: watt@uwo.ca. CC: hong@math.ncsu.edu.

Dear Professor Giorgetti,

This is to inform you that your revised paper 

    "Rewriting and symbolic transformations for multiscale methods"

(JSC YJSCO-7601) by Belkir et al.  has been accepted for publication.

Your responses were forwarded to the original reviewers together with the the
revised paper and the software package you provided.

The editor-in-chief is in receipt of a copy of this message and you will receive
information on how to provide the required materials for the publication.

I do apologize for the length of time that it has taken to come to this
conclusion, and for not being more responsive throughout the process.

Sincerely,

Stephen M. Watt, PhD, DSc h.c., ICD.D,
Distinguished University Professor,
The University of Western Ontario.

\subsubsection{Submission message}
Date: 16/11/2011.

To: smwatt@gmail.com, koepf@mathematik.uni-kassel.de

Cc: walid.belkhir@lifc.univ-fcomte.fr, michel.lenczner@utbm.fr

Dear Professors Koepf and Watt,

In my last message (attached) I expected to submit a revision of our paper 

 Rewriting and Symbolic Transformations for Multiscale Methods

before the end of June. 

Unfortunately our will to fulfill strong quality requirements 
and to provide a fully operational software have delayed our
submission up to now. Please apologize for the delay.

We are now honored to submit to JSC an extension of that paper, now
entitled ``A Symbolic Transformation Language and its Application
 to a Multiscale Method''. This submission is the attached file BGL.pdf. 

We accompany this submission with one answering letter for each referee
of the former paper (attached files \url{for_reviewer_1.pdf} and
\url{for_reviewer_2.pdf}) and an archive containing the current version of
the software described in the paper (file symbtrans.1.0.zip). After
extraction, reading the file readme.txt and the paper BGL.pdf provide
to a Maple user all the necessary information to use the package. 

We would greatly appreciate if you could transfer these answers and this
software to the referees.
Best regards,

> Thank you for the referee reports and the invitation to submit to JSC.

> We are taking the referee's comments into account and plan to submit
 an enriched version of our article

>   Rewriting and Symbolic Transformations for Multiscale Methods

> before the end of June.

Best regards,

AG, 20/07/2012: Dear Professors Koepf and Watt,

On November 16, 2011, I submitted to the Journal of Symbolic Computation a joint
paper with M. Lenczner and W. Belkhir, entitled "Rewriting and Symbolic
Transformations for Multiscale Methods", by sending you the attached message.

I am coming back to you because since that date we have not received any news
about this submission.

Could you please inform us about the current status of our submission? Does the
Journal of Symbolic Computation use the Elsevier Editorial System (EES)? If yes,
how can I follow the status of our paper?


SW, 16/08/2012: Dear Prof Giorgetti,

I apologize for taking some time to reply.  I have been on family
vacation and will be returning to the office next week, at which point
I should be able to give some details.

Yours,

Stephen

\subsubsection{Submission conditions}
It is strongly recommended that the paper is prepared in LaTeX using the
"Elsevier Article Class (elsart.cls)" with "JSC add-on style (yjsco.sty)" and
"Harvard style references (elsart-harv.bst)". This will significantly speed up
the publication process of the paper. The package "JSC LaTex" (that contains all
the necessary style files and a template) can be obtained from here.
Send an email to the Editor-In-Chief (Prof. Hoon Hong, hong@math.ncsu.edu) with
the following content:

1. The title of the paper.

2. For each author, the name and the postal address.

3. The abstract (must be a plain text).

4. The names of three editorial board members whom you suggest to "organize" the refeering of the paper. Make sure:

          * that the persons are expertson the subject of the paper and

          * that there is no conflict of interests between you and the suggested editorial board members.

      Usually, one out of the three will be chosen to organize the review of the paper.

5. Attach the paper (must be in either "pdf" or "postscript" format)

\subsection{ISSAC 2010 JSC special issue}
Corresponding author : Alain Giorgetti.

JOURNAL OF SYMBOLIC COMPUTATION,
SPECIAL ISSUE ON SYMBOLIC AND ALGEBRAIC COMPUTATION,
FOUNDATIONS, ALGORITHMICS AND APPLICATIONS.

Guest Editors: Wolfram Koepf and Stephen M. Watt.

This special issue is related to topics discussed in the context of
the ISSAC Conference in July 2010 in Munich, Germany.

\subsubsection{Submission message}
From: AG, 10/12/2010. To: koepf@mathematik.uni-kassel.de. Cc:
Stephen.Watt@uwo.ca:

Dear Editors,

Enclosed is a PDF file of an article entitled "Rewriting and Symbolic
Transformations for Multiscale Methods" that my co-authors and I are submitting
for publication in the special issue of the Journal of Symbolic Computation
related to topics discussed in the context of the ISSAC Conference in July 2010
in Munich, Germany. Best regards,

\subsubsection{Rejection message}
Stephen Watt, 23/05/2011: Dear Professors Giorgetti and Belkhir,

The review process for the JSC Special Issue is now mostly complete.
I apologize for not being able to send the results earlier.

Based on the referee reports, we have concluded that your article

    Rewriting and Symbolic Transformations for Multiscale Methods

will not be included in the special issue.   As both of us (the
special issue editors) are also members of the editorial board of JSC,
however, we we would like to consider your article as a regular
submission to the journal.

Please find attached the anonymous form of two referee reports.   If
you wish to proceed with your article as a regular submission, please
send us a revision taking the referee's comments into account.

\subsubsection{Referee reports of JSC special issue}

\paragraph{Referee 1}
\begin{small}
\begin{verbatim}
Journal of Symbolic Computation
   Referee Report Form

Paper Identification
--------------------
JSC ID         : JSC-ISSAC10-06
Title          : Rewriting and Symbolic Transformations for Multiscale Methods
Author Name    : Walid Belkhir and Alain Giorgetti and Michel Lenczner
Tutorial (Y/N) : N 


Judgement
---------
  (1 Excellent;  2 Good;  3 Average;  4 Below Average;  5 Poor)
 
  * Relevance to the field of symbolic computation     : 2
  * Originality (does not apply to tutorial papers)    : 2
  * Importance, significance and value of contribution : 3
  * Logical and formal correctness                     : 2
  * Proper crediting/citing of previous literature     : 1
  * Clarity, structure and style of presentation       : 2
  * English grammar/spelling                           : 4

  Recommendation (Accept/Revise/Reject) : Accept


Comments to the author
----------------------

The paper concerns a Maple package `symbtrans', written by the authors,
intended to provide a facility for implementing rewriting rules within Maple.
The package purports to provide better user control than the extand facilities
already provided [[AG: extand?? patmatch and subs?]].  The authors indicate that
a significant shortcoming of the applyrule facility in Maple is that it does not
 allow for function symbols to
appear as pattern variables [[AG: a matter of encoding, do not emphasize? ]], a
problem which their symbtrans package solves. They also give, by way of example,
 a significant application of their package
to a formalised proof of a "gradient weak convergence" result, effected by
means of a two-scale transform.

The paper is a nicely written, apparently original contribution.  While the
authors propose no theoretical advance (they are building on theoretical
formalisms already present in the literature), the engineering contribution,
and its application to the important field of multi-scale methods in modeling,
deserve attention.  There are, in addition, some nice ideas proposed in the
Maple implementation.

There are a few comments on the content of the paper, as follows.

1.  The definition of the TopDown transform (p. 8) does not seem to be as
efficient as it could be.  Unless I've misunderstood something, perhaps
something like the following might be better (allowing for plain text
notation)?

------------------------------------------------------------------------
TopDown(s)(t) = if t = t'(t_1,...,t_n) then
	u := FailAsIdentity( s )( t );
	if u = t then
		u
	else
		t'( TopDown( s )( t_1 ), ..., TopDown( s )( t_n) )
------------------------------------------------------------------------

[[ Oui pour la factorisation de l'application de s à t.
s(t) or FailAsIdentity(s)(t) ? (partout, sémantique ?) u = t efficace ?
Maximal sharing? TODO 2, AG, 2 days: test in Maple. TODO 3, WB, 1 day: Discuss
complexity issues. ]]

2. The FreshIndex() mechanism for distinguishing various copies of "BigO" is
obviously workable, but seems to complicate the notation considerably.  There
are two other *possible* solutions the authors might explore.

The first is to use generated local names for the name `O'.  Since these local
names differ, automatic simplification to 0 will not occur.  Such local names
can be generated by using the Maple procedure `tools/gensym`.  For example,
in Maple we'd get:

> > u := `tools/gensym`( O )( e );
                                   u := O(e)

> > v := `tools/gensym`( O )( e );
                                   v := O(e)

> > u - v;
                                 O(e) - O(e)
[[WB: One of the  problems of this solution is that writing a convergence strategy
 with this technique is not possible for many reasons:

> r:=[`tools/gensym`( O )( e )+ `tools/gensym`( O )( e ),`tools/gensym`( O )( e )];    
                      r := [2 O(e), O(e)]

Besides, the following matchings fails, ours and that of Maple:

>  Matching(`tools/gensym`( O )( e ),`tools/gensym`( O )( e ));
   Error, (in Matching2) Fail

> patmatch(`tools/gensym`( O )( e ),`tools/gensym`( O )( e ))
   false
 
]]


A second possibility is to use attributes on the unevaluated function calls.  
For example,

> > u := setattribute( O(e), 1 );
                                   u := O(e)

> > v := setattribute( O(e), 2 );
                                   v := O(e)

> > u - v;
                                  O(e) - O(e)

This has the effect of producing two apparently identical `O(e)' expressions,
but which are, in fact, different due to the presence of attributes.

These two alternatives are, obviously, isomorphic to the solution presented in
the paper, but might provide a nicer notation.  (It's also possible one or the
other might introduce complications that I cannot foresee without attempting a
full implementation.  These are meant only as suggestions for further study.)


[[ TODO 3, WB, 1 day: Se renseigner sur ces fonctionnalités Maple. TODO 4,
WB and AG, meeting: Decide to use them or not (answer to referee). TODO
5, WB, 1 day: Replaced by backquote or DelayEval (argument pour : similaire à Mathematica). 
DONE 6, AG : no problem with DelayEval in a Maple module. ]]

3.  I have not thought this through too carefully, but the authors might
investigate the use of the `::uneval' parameter modifier as an alternative to
the `EvalRule' construct.  Both seem to be designed to solve the same sort of
problem, and the fact that the semantics of `::uneval' are builtin to the Maple
kernel might allow for a more efficient implementation (if it can be made to
work in this context).

[[ TODO 6, AG, 1 day: Se renseigner sur cette fonctionnalité Maple. TODO
7, AG and WB, meeting: Decide to use it or not (answer to referee). ]]

[[ DONE 1 ]] Many suggested (minor) corrections to the English follow (page,
paragraph and line number, or numbered/titled item).

4. In the code that appears in Appendix B, there are a number of occurrences of
evala@Expand.  The need for these should be explained somewhere in the text of
the article, as they are likely to seem quite mysterious to someone not
intimately familiar with Maple.

Page 2:

para 1, line 3:

	- comma after "etc.".
para 2, line -3:

	- The word "orient" does not seem right here.  Presumably, you mean
	  that an equation "x=y" represents a rewrite rule "x -> y".

para 4, line 2:

	- The word "imposed" is probably not right; it has a negative
	  connotation, as though you meant you were forced to use Maple against
	  your will.

para 4, line -4:

	- semicolon (:) after "flexibility".

Page 3:

para 1, line 1:

	- The fragment "we give a good amount" is awkwardly worded. Perhaps you
	  could use something like: "In this work, we provide a significant
	  rewriting feature for Maple."

para 4, line 4:

	- "give" --> "giving"

para 5, line 3:

	- "no more rule" --> "no more rules"

para 5, line 4:

	- "no more rule" --> "no more rules"

Page 4:

para 3, lines 1-2:

	- insert commas after "And" and before "where":
	"And if t_1 ... then t(t_1,...,t_n) \in T(F,X) where"
	--> "And, if t_1 ... then t(t_1,...,t_n) \in T(F,X), where"

para 7, line 1:

	- "It is worth to mention that" --> "It is worth mentioning that"

para 9, lines 1-2:

	- "equation" --> "equations"

para 9, line 2:

	- "physical modelings" --> "physical models"

para 9, line 7:
	
	- Should "in the n directions" read "in the n orthogonal directions"?

para 8, line 8:

	- "In view to derive the" --> "With a view to deriving the"

Page 5:

para 1, line 3:

	- This should probably be restyled as a proper reference indicating
	  whether the stated authors originated or exposed the variational
	  form. 
	
	      "written in its variational form Dautray and Lions (1990)."

	   --> "written in its variational form, due to Dautray and Lions (1990)."
	   or
	   --> "written in its variational form, as explained in Dautray and Lions (1990)."
	   or
	   --> "written in its variational form (see Dautray and Lions (1990))."

para 2, line 3:

	- "a process called two-scale transform" --> "a process called a two-scale transform"

para 2, line 10:

	- "we end to" --> "we arrive at"

para 2, line -2:

	- "for all v0 sufficiently regular test function vanishig on"
	   --> "for all sufficiently regular test functions v0 vanishing on"

para 3, line 1:

	- "approximated" -->  "approximate"

para 3, line 2:

	- start new sentence: "Lenczner (1997) then" -> "Lenczner (1997). Then"

para 3, line 9:

	- "The two first consist in" --> "The first two consist of"

para 3, line 11:

	- "yields" --> "yield"

para 3, line -2:

	- "so to be used" --> "so can be used"

para 4, line 1:

	- "Before to state the property" --> "Before stating the property"

para 4, line 2:

	- "in" --> "on" (i.e., on Theta)

para 4, line 3:

	- insert comma after "that is"

para 4, line -1 (i.e., last line of p. 5):

	- "oposite" --> "opposite" (spelling) 

Page 6:

para 1, line -1:

	- "gradient" --> "gradients"

Proposition 3, line -3:

	- insert commas before and after "respectively"

para -2, line -5:

	- "it always do not" --> "it always does not"

para -2, line -2:

	- "by" --> "but"  (before "it exceeds the scope")

Page 9:

para 1, line -2:

	- "distinct of t" --> "distinct from t"

para 2, line 2:

	- "most of the programming languages" --> "most programming languages"


Page 10:

para -1, line 1:

	- "until no more v is under a div operator" should be re-worded as
	  something like "until v is no longer under a div operator"

Page 11:

para 1, line 2:

	- "so that to get" --> "so as to get"

para 4, line 3:

	- there seems to be an extraneous backslash in "r\_epsilon" (should it
	  be "r_epsilon"?)

para -1, line 1:

	- "has been already" --> "have already been"

Page 13:

para 3, line -1:

	- "requires a separated work" --> "requires a separate work"

Page 14:

para -1, line 5:

	- "learns it quickly, is free to" --> "learns it quickly, and is free to"

Page 15:

para -2, lines 2-3:

	- I'm not certain, but it looks as though TeX quotes (``level'') should
	  be used, where double quotes ("level") appear around the word `level'.

Page 16:

para 1, line 1:

	- "guarantee the correction" --> "guarantee the correctness"

para 1, line 3:

	- The word "work" is slightly awkward, and it may be better to use
	  something like "project".

Page 17, et seq:

	- The dot (.) operator seems to be used inconsistently throughout Appendix A.

Page 17:

Lemma 8, line 1:

	- "at the zero order" --> "at order zero"

Lemma 9, line 1:

	- "at the zero order" --> "at order zero"


Page 18:

Step 3:

	- "and it remains" --> "and it follows that" (or similar)

Step 4:

	- In the formula (ASCII approximation) "div(Bv) = B div_x v + 1/epsilon
	  B div_y", there seems to be a "v" missing from "div_y v".

Step 5:

	- "at the zero order" --> "at order zero"

Step 7:

	- "we use assumptions" --> "we use the assumptions"

Page 19:

Step 8:

	- "and it remains" --> "and we obtain" (or similar)

Step 9:

	- How did the Stieltjes integrals suddenly appear?

\end{verbatim}
\end{small}

\paragraph{Referee 2}
\begin{small}
\begin{verbatim}
               Journal of Symbolic Computation
                    Referee Report Form

Paper Identification
--------------------
JSC ID         : 
Title          : Rewriting and symbolic transformations for multiscale methods
Author Name    :  Belkhir at al.
Tutorial (Y/N) :  N


Judgement
---------
  (1 Excellent;  2 Good;  3 Average;  4 Below Average;  5 Poor)
 
  * Relevance to the field of symbolic computation     : 2
  * Originality (does not apply to tutorial papers)    : 3
  * Importance, significance and value of contribution : 3
  * Logical and formal correctness                     : 2
  * Proper crediting/citing of previous literature     : 3
  * Clarity, structure and style of presentation       : 4
  * English grammar/spelling                           : 3

  Recommendation (Accept/Revise/Reject) : Revise


Comments to the author
----------------------

The authors present a number of claims without proof. 
[[ DONE 8, WB, 2 days: Turn these claims into clear contributions and justify 
their interest. ]]
 
Specifically, they claim to have 
devised and implemented a new pattern matcher in Maple. At first reading, they appear to be
claiming only to port existing pattern matching to Maple, although on re-reading 
they appear to have
grounds for claiming more. [[ DONE 8 also: More? All the solutions, for
conditional rewriting rules. AC-matching? ]]

The real problem is the fact that they describe only the functions and the
calling sequences of their package. How can I get this package and try out their code?

[[ TODO 9, AG, 5 days, in a footnote
in the paper, then WB, 5 days: Maple cloud? No. Help
pages, package, user manual, examples, testing, code cleaning, download. ]]
 
The application of their system is left mostly to an appendix. Here I see very little description of 
automatic application. Transformations are described and implemented, 
leading to the desired result, but the derivation is done step by step. 
Thus the re-write rules allow a user
to cunduct a calculation with greater accuracy and ease,
 but each step is still user decided and directed.

[[ TODO 10, AG, 2 days: Study and present the addition of some automation in the
gradient proof. Initiated in rewriting/GradientProof/normal.mpl.]]

I would be happy to recommend this paper if it allowed be to use their system in my own work, 
but the present version does not allow this. The paper should not be a complete user manual, but it should
combine a discussion of theoretical fundamentals [[ TODO 11, WB, 3 days: What is
the underlying ``strategy calculus''? Reducible to rho-calculus. Why not implementing 
the rho-calculus? Strategies less efficient. ]] with practical information such as download possibilities
[[ TODO 9 also.]].
\end{verbatim}
\end{small}

\subsubsection{Answer to ISSAC referees}
In the files \url{for_reviewer_1.tex} and \url{for_reviewer_2.tex}.

On a suivi toutes les recommandations des relecteurs.

Par rapport à l'article précédent, on a ajouté : conditional rewrite rules,
blocage d'évaluation général, deux preuves au lieu d'une (indices et sommes pour
éliminer le gradient et le produit scalaire).

DONE 12, WB, 2 days, lié au TODO 11 : Réviser l'introduction : présenter mieux
uniformisation des méthodes multi-échelles. Ajouter références sur calcul
symbolique avec réécriture. Insister sur les contributions : contextual
rewriting, multi-paradigmes. 
Discuter le choix de Maple : avantages / inconvénients.
On utilise de plus en plus des features Maple (uneval, fonctionnalités
impératives efficaces, maximal sharing). Comparer avec Maude.

DONE 13, WB, 2 days : conditional rewrite rules, blocage d'évaluation
général.

DONE 14, WL: Include the diffusive equation example.
Confidentiality.

DONE 16, WB, 1 day. Related work: Read \cite{KMR06}, \cite{BKK+99} and Section 4
in \cite{BBK_Tom07} and compare with our work. rholog, Elan.

\subsection{Pretty-printed proof output}
\label{proof:pp:sec}
Le fichier \url{paper/JSCspecial11/GradientProof/gradientPP.tex} inclus
ci-dessous est produit par le code Maple \texttt{postprocess.mpl}. Le résultat
n'est pas d'assez bonne qualité pour être inclus dans l'article.

\input{paper/JSCspecial11/GradientProof/gradientPP.tex}

\subsection{Removed text}

Now we start from a simple problem \[ \left\{
\begin{array}{c}
-\func{div}(a^{\varepsilon }(x)u^{\varepsilon }(x))=f^{\varepsilon }(x)\text{
in }\Omega \\
u^{\varepsilon }(x)=0\text{ }on\text{ }\partial \Omega%
\end{array}%
\right.
\]%
to explore the method of automatic derivation of TST model%
\[
\int_{\widetilde{\Omega }}(\nabla _{\widetilde{x}}u^{0})^{T}\left[
\int_{Y}a(I+\mathcal{L})^{T}(I+\mathcal{L})dy\right] \nabla _{\widetilde{x}%
}v^{0}d\widetilde{x}=\int_{\widetilde{\Omega }}\left[ \int_{Y}f^{0}dy\right]
v^{0}d\widetilde{x}
\]%
. [[ AG: take less place to present the equations above and please explain the
notations. ]]

\subsection{Abstract}
\label{about:jsc:abstract:sec}
Pas de police spéciale pour écrire ``MEMSALab'', comme dans EuroSimE-2011.

\subsubsection{Removed sentences}
The challenge is to formalize these approximating methods within a computer
algebra system, e.g. Maple$^{\text{\textsf{\tiny TM}}}$. Our contribution
consists in transferring most of the term rewriting concepts and techniques to
the symbolic computation community.

Since most of the transformation steps correspond to equational reasoning
(i.e. symbolic transformations based on equalities) we address the 
question of extending Maple$^{\mathsf{TM}}$ with rewriting and strategies.

\subsection{Introduction}

\subsubsection{Phrases ôtées, à replacer ?}
The produced simulations should be light enough to be inserted into parameter
identification and optimization loops.


Another drawback is that there is no straightforward way to rewrite
terms with variable function symbols (we would like to write $f{\_}(...)$
where $f{\_}$ is not a fixed symbol but a variable that ranges over a set of
function names).


Such  functions can be combined to define higher-order strategies.

(à reformuler avant. ML : pas terrible)  Thanks to the ability of the host
language Maple$^{\mathsf{TM}}$ to perform functional programming, our
 transformation language is built up from a functional point of view.

(ML : me paraît bien optimiste ! Il faudrait être plus précis dans cette annonce
marketing) The transformation steps involved in this particular case are general
enough to be applied to much more complicated models. This good level of
generality is reached thanks to the powerful transformation combinators provided
by \ST.


(à placer en début de partie 5) This section explains the notations used in the
formal proofs and introduces a computational version of the notion of
convergence -- in the sense of  the two-scale transform -- and its properties.
Some problems  related to the evaluation strategy of
 Maple$^{\mathsf{TM}}$ are pointed out and solved. 

\subsubsection{Removed sentences}
A great challenge is to generalize these formal computations and to automate them.
(supprimé car détaillé plus loin).

From the point of view of geometric features, the MEMSALab software  we
develop aims at filling this gap. In fact, it will aid to design 
multiphysics systems with high contrast in equation coefficients and complex 
geometries including thin structures, periodic structures with possibly many 
nested scales, and combinations of these. (supprimé car dit plus loin)



The  model under study might be viewed as an \emph{equational system}. We are
interested in knowing if a given equation  can be derived from such a system.
The final equation is given either in an explicit way or in terms of a more general
pattern.

\ldots when describing,  by means of inference rules, a logic, a theorem prover
or constraint solver.
\subsection{Preliminaries and notations}
File \url{rewrite.tex}.

\subsubsection{TODO}

``Further clarifications on this topic can be found in Section
\ref{package:sec}.'' Where? Peut-on éviter ce renvoi ?

Revoir la phrase définissant la confluence, pas assez précis.

La définition actuelle de l'application d'une règle de réécriture à un terme est
: ``The \emph{application} of a
rewrite rule $\rrule{l}{r}$ to a term $t$, denoted by $[\rrule{l}{r}](t)$, is
defined by $\sigma(r)$ where $\sigma$ is a solution of the matching
$\match{l}{t}$.'' Dans cette phrase, le ``a solution'' laisse supposer qu'il
peut y en avoir plusieurs. Dans ce cas, laquelle choisir pour calculer
$\sigma(r)$ ? Pour que cette ``définition'' en soit vraiment une, il reste à
expliquer ou affirmer que toutes les solutions donnent le même résultat.

Définir l'application d'une substitution à un terme, au moins informellement,
ou supposer connu, explicitement.
AG (pour ML): ``The proof is organized in four parts.'' Dommage qu'on ne
retrouve pas ces quatre parties explicitement dans les annexes.
Ajouter $x = x_1, \ldots, x_n$, dans $\Omega$ ou $\macrodom{\Omega}$ et $y =
y_1, \ldots, y_n$, dans $Y$, pour qu'on comprenne d'où viennent les $x_i$ et les
$y_i$.
 
Ajouter une référence aux annexes mathématiques dans example.tex ?

AG (pour ML): Revoir l'énoncé de la proposition 3 : Que veut dire ``formal
expansion'' ? Il y a un risque de confusion avec le calcul formel. Ajouter une
phrase pour introduire cette proposition. Cette phrase peut être ``The following
proposition has been introduced [Peut-on citer un article ici ?] as an
assumption in the statement, to simplify the proof.'' et elle peut remplacer  la
phrase ``We observe that the expansion (\ref{Expansion of Tu}) has been 
introduced as an assumption in the statement, to simplify the proof.'' qui suit
la proposition.

\subsubsection{Remarques}
ML : ``constant'' Ambiguité avec les constantes pour linéarité ?
Je ne suis pas certain qu'il y ait une réelle différence avec les
maths [à propos des constantes] de ce point de vue là.

AG : Résolu : Clairement expliqué après l'exemple 2.

WB : Pour la linéarité, on parle de ``scalaire''.

AG : On définit ici les règles de réécriture du premier ordre, mais dans la
partie 4 on permet d'écrire des règles plus générales, avec des lambda-termes en
partie droite.
 
ML, running example, proposition 3 : Il faudrait savoir justifier pourquoi cette
simplification a été faite, si on peut la supprimer ou si on peut justifier
qu'avec la théorie actuelle on ne peut pas l'atteindre. \mycomment{ML}{We can do
better.}

AG : C'est un travail mathématique à faire séparément. Ici, on peut demander au
lecteur d'admettre, en disant que cela correspond à la preuve actuelle. Puis,
dans les perspectives, on peut dire qu'en formalisant ainsi on espère aussi
prouver mieux ou plus de choses, par exemple se passer de cette simplification.

ML : Met en oeuvre que la fonction test $v$ est périodique. Comme on n'a pas
encore typé les fonctions, on ne peut pas formaliser cette preuve.

AG : Voir si la définition de la linéarité ne serait pas mieux dans la partie 4.
 
\subsubsection{Removed sentences}
 If $x\in \mathcal{X}$ then $x\in \mathcal{T(F,\mathcal{X})}$.
And, if $t_1,\cdots t_n \in \mathcal{T(F,\mathcal{X})}$ are terms, then \ldots
(reformulé).
  
``problem of partial differential equations, namely the diffusive equation. It
appears in a number of physical models  such as the heat equation, the equation
of electrostatics, the model of thin elastic beam in torsion, etc.'' (restreint
à la ``stationary heat equation'' dès le début).


\subsubsection{Example}
Dans le fichier example.tex. Cette partie donne un exemple de mod\`ele
math\'ematique qu'on transforme. Ce mod\`ele vient de [Lenczner08], pages
22--24. Dans l'expos\'e talk/LTP10/, on a pr\'esent\'e le mod\`ele
math\'ematique comme suit :

Le probl\`eme physique est formul\'e en termes d'\'equations diff\'erentielles :

\begin{align*}
\left\{
\begin{array}{c}
 - div(a^{\varepsilon }(x)u^{\varepsilon }(x))=f^{\varepsilon }(x)\text{
dans }\Omega \\
u^{\varepsilon }(x)=0\text{ }  \text{ sur } \partial \Omega
\end{array}%
\right.
\end{align*}
avec $\varepsilon=\frac{L}{n}$. Extension au domaine produit $\Omega \times Y$.
Approximation $\tilde{u}$ du champ et approximation
\begin{equation}
\int_{\omega}(\nabla _{\widetilde{x}}u^{0})\left[
\int_{Y}a(I+\mathcal{L})(I+\mathcal{L})dy\right] \nabla _{\widetilde{x}%
}v^{0}d\widetilde{x}=\int_{\omega}\left[ \int_{Y}f^{0}dy\right]
v^{0}d\widetilde{x} \label{model:diffusion:approx:eq:french}
\end{equation}
du mod\`ele, quand $n \rightarrow \infty$, i.e. quand $\varepsilon \rightarrow
 0$. Ici je sugg\`ere qu'on commence directement par la formulation
 variationnelle, ce qui donne : ]]



Let us consider the example
\begin{equation}
\int_{\Omega} -div(a^{\varepsilon} \nabla u ^{\varepsilon})  v dx =
\int_{\Omega} f^{\varepsilon} v dx
\label{model:diffusion:variational:eq:french}
\end{equation}
of the variational formulation of the diffusion equation on the domain $\Omega$.
In this equation, $u$ is\ldots

[[ Alain, pour Michel: pourrais-tu compl\'eter ici la description de ce
mod\`ele, stp ? Voici nos questions \`a ce sujet :

1. Pour comprendre cette \'equation, j'ai consult\'e wikipedia
(\url{http://en.wikipedia.org/wiki/Diffusion_equation}). Ces deux d\'efinitions
de l'\'equation de diffusion correspondent, selon la correspondance $r
\rightarrow x$, $D(r) \rightarrow a^{\varepsilon}(x)$, $\phi(r,t) \rightarrow u
^{\varepsilon}(x)$, sauf le terme $f^{\varepsilon}$ dont je ne comprends pas le
lien avec $\dfrac{d\ \phi(r,t)}{dt}$. Peux-tu stp enrichier ce fichier avec une
explication ``self-contained'' du contenu de cette \'equation et de son sens
physique ? Remarque que la formulation variationnelle ci-dessus n'est pas celle
de ton document, mais il me semble qu'on l'obtiendrait par une application de la
formule de Green. Je propose qu'on explicite ici cette \'etape, en tant
qu'exemple de raisonnement \'equationnel/r\'e\'ecriture. ]]

\subsubsection{Archive}
J'ai remplacé partout les terminologies et notations ``math\'ematiques'' comme

\bigskip

``$y\mapsto a(y)$ is defined in $\mathbb{R}^{n}$''

\bigskip

par une notation plus ``informatique'', o\`u l'on voit le ``type'' des
fonctions math\'ematiques. Par exemple,

\bigskip
``The diffusion
coefficient is assumed to be rapidly varying in space. Precisely, we assume
that it is periodic, with a small period $\varepsilon ,$ in the $n$
directions: $a^{\varepsilon }(x)=a(x/\varepsilon )$ for $x\in \Omega ,$
where $y\mapsto a(y)$ is defined in $\mathbb{R}^{n}$ and is $(0,1)^{n}$%
-periodic.''

is replaced by

``The diffusion coefficient $a^{\varepsilon} : \mathbb{R}^{n} \rightarrow
\mathbb{R}$ is assumed to be periodic on $\Omega$ in the $n$ directions,
with a small period $\varepsilon$. This means that there is a function $a :
\mathbb{R}^{n} \rightarrow \mathbb{R}$ which is $(0,1)^{n}$-periodic and
such that $a^{\varepsilon}(x)=a(x/\varepsilon)$ for $x\in \Omega$.''

\bigskip

De m\^eme, on remplace $x\mapsto f^{\varepsilon}(x)$ par $f^{\varepsilon}
$ et $x\mapsto u^{\varepsilon}(x)$ par $u^{\varepsilon}$, $x\mapsto v(x)$
par $v$ et on en profite pour préciser leur ``type''.

\bigskip

\textbf{Pour Alain: }\textit{Dans le lien wikipedia que tu m'as donné, il
s'agit d'une équation de diffusion non stationnaire sans terme de source }$f$%
\textit{. Le terme }$d\phi /dt$ \textit{est la dérivée par rapport au temps
qui apparait dans l'équation d'évolution et qui est absent dans l'équation
du phénomène stationnaire. Concernant la formulation variationnelle, c'est
celle qui est écrite dans le document qui porte ce nom là. Celle que tu as é%
crite est équivalente mais n'a pas de nom particulier (il s'agit
effectivement d'une étape intermédiaire entre la formulation forte et la
formulation faible (ou variationnelle) et elle ne sert à rien. }

[[ Alain, pour Michel : ainsi r\'edig\'e, c'est clair pour le second membre.
Concernant la forme variationnelle/faible, il me semblait que
l'\'equivalence entre ma formule et la tienne s'obtenait par la formule de
Green. Peux-tu confirmer, stp ? Si oui, n'a-t'on pas besoin d'une condition
du nullit\'e sur les bords pour obtenir cette \'equivalence ? J'aimerais
bien lire cette preuve d\'equivalence. A quelle page de \cite{DauLio}
est-elle ?

Un point technique : Lorsqu'une discussion dans cette r\'edaction est close,
on ne l'efface pas mais on la d\'eplace dans about.tex. ]]

\bigskip

[[Michel: Tu peux appeler formulation variationnelle. L'équivalence
s'obtient par la formule de Green en tenant compte du fait que $v=0$ au bord
(ce que j'ai indiqué) mais par contre on n'a pas besoin d'hypothèse sur $u$
au bord. Je ne sais pas où se trouve la démonstration dans Dautray Lions (je
ne l'ai pas avec moi) tu peux également la trouver dans le livre de Raviart:
"Introduction a l'analyse numerique des equations aux derivees partielles"
de chez Masson dans les pages 41-43. Tu peux le télécharger ici
http://gen.lib.rus.ec/search?req=raviart\&nametype=orig]].


Alain : c'est clair. J'ai remplacé partout ``weak form'' par ``variational
form''.


Let $u^{0}$ be the limit of $u^{\varepsilon }$ when $\varepsilon $ decreases
to zero. It can be shown that $u^{0}$ is the unique solution to the equation
\begin{equation}
\int_{\omega }(\nabla _{\widetilde{x}}u^{0})\left[ \int_{Y}a(I+\mathcal{L}%
)(I+\mathcal{L})dy\right] \nabla _{\widetilde{x}}v^{0}d\widetilde{x}%
=\int_{\omega }\left[ \int_{Y}f^{0}dy\right] v^{0}d\widetilde{x}
\label{model:diffusion:approx:eq:too:complex}
\end{equation}%
where \ldots

[[ Alain, pour Michel : Pourrais-tu stp compléter ici en expliquant ce que
sont $\tilde{x}$, $v^{0}$, $I$, $\mathcal{L}$, etc. Il ne s'agit pas
d'expliquer toute la théorie, mais juste de préciser la nature de ces
grandeurs et comment elles dépendent des données. ]]

[[Michel: Ca ne semble pas utile de donner cette formulation avec ce niveaud
de détail, dans la mesure où on ne l'établit pas. Il suffirait de donner la
formule finale avec $a^{H}$ à la place de $\int_{Y}a(I+\mathcal{L})(I+%
\mathcal{L})dy$. Idem, je ne vois pas l'intérêt d'introduire les $\omega $
et $\widetilde{x}$ plutôt que $\Omega $ et $x$. Idem pour le second membre.
Au total, il suffirait d'énoncer le modèle final%
\begin{equation*}
\int_{\Omega }(\nabla _{x}u^{0})a^{H}\nabla _{x}v^{0}dx=\int_{\Omega
}f^{H}v^{0}dx
\end{equation*}%
en précisant simplement qu'ici le coefficient $a^{H}$ n'est pas oscillant.
Dis moi si ça te convient?

Alain : ce modèle plus simple me convient. J'ai modifié. Il reste à expliquer ce
qu'est $a^{H}$, et à distinguer les produits scalaires multidimensionnels par
un point. ]]

\subsection{Transformation language}

\subsubsection{\texttt{STNormalizer}}
La notion classique de \emph{forme normale} concerne la réécriture en profondeur
quelconque, en toute position, pas seulement à la racine. En ce sens,
\texttt{STNormalizer} ne calcule pas toujours une forme normale, comme le montre
le test[7] dans regtest.mpl, qui se résume à :
\begin{verbatim}
 r := [a,b];
 t := f(a);
 t2 := STNormalizer(FailAsIdentity(r))(t);
 printf("STNormalizer(%a)(%a) = %a is not the normal form f(b).\n",r,t,t2);

 if not ( t2 = f(a) ) then
  nbError := nbError + 1;
 fi;
\end{verbatim}

Le nom \texttt{STNormalizer} est donc mal choisi pour cette fonction.

Ce qu'on a écrit dans dMEMS'2012 à ce sujet n'est pas correct non plus.

En Tom, l'itération est possible avec \textit{Repeat} et \textit{RepeatId}.

\begin{eqnarray}
\textit{Repeat}(s) & = & \mu x. \;
    \textit{Choice}(
      \textit{Sequence}(s,x),\textit{Identity}) \\
\textit{RepeatId}(s) & = & \mu x. \;
      \textit{SequenceId}(s,x)
\end{eqnarray}

Au 13/11/2011, je n'ai pas terminé la comparaison formelle entre ces fonctions
et \texttt{STNormalizer}, mais mes premiers essais me donnent l'impression
qu'elles ne coïncident pas. 

Les nouvelles définitions de TopDown et BottomUp ont plus d'effet que
\texttt{STNormalizer}. Elles peuvent probablement être utilisées à sa place dans
toutes les preuves actuelles. Malheureusement, je n'ai pas le temps de le
vérifier. Comme beaucoup de code et de documentation utilise déjà cette
fonction, on la maintient, mais elle nécesssite une étude plus approfondie.
 
\subsubsection{TODO}
\paragraph{LeftChoice failure}
Le choix parmi $n$ transformations doit-il échouer si aucune ne s'applique ? En
pratique (critère principal), on préfère qu'il n'échoue pas. Mais, en théorie,
on préfère disposer des constructeurs de stratégies les plus fins possibles,
pour ne pas se priver d'un moyen plus précis de spécifier. Ceci justifie le
choix
\begin{displaymath}
\begin{array}{|r l|}
\hline
\texttt{LeftChoice([\,])(t)} &=_{\textit{def}} \texttt{Fail(t);} \\
\hline 
\end{array}
\end{displaymath}
au lieu de
\begin{displaymath}
\begin{array}{|r l|}
\hline
\texttt{LeftChoice([\,])(t)} &=_{\textit{def}} \texttt{t;} \\
\hline 
\end{array}
\end{displaymath}
En effet, à partir du premier, noté \texttt{LC1} ci-après, on peut
facilement coder le second, ci-après noté \texttt{LC2}, par exemple par
% \footnote{TODO: put
% here the right Maple syntax to add an element at the end of a list.}
% \begin{displaymath}
% \begin{array}{|r l|}
% \hline
%  \texttt{LC2(l)} & = \texttt{LC1([op(l),Identity])}\\
% \hline
% \end{array}
% \end{displaymath}
% ou plus simplement par
\begin{eqnarray*}
\texttt{LC2} & = & \texttt{FailAsIdentity}(\texttt{LC1}),
\end{eqnarray*}
tandis que le contraire est plus difficile à exprimer. On a modifié \ST ainsi.

Pour modifier le moins possible l'implantation, les annexes et les théories,
on met aussi \texttt{LC2} à disposition de l'utilisateur de \ST,
et on l'utilise pour coder Outermost et Innermost.
\paragraph{Forme normale}
La notion de forme normale est définie pour une règle de réécriture, et plus
généralement pour un système de réécriture ``sans priorités'' [ TODO : Voir le
nom ``officiel'' dans TeReSe. ]. Avant de parler de forme normale pour une
stratégie/transformation, il faut étendre cette notion, si possible. L'exemple
$$\texttt{STNormalizer}(LeftChoice([[b,c],[a,d]])(a),$$ qui échoue, montre qu'il
faut bien envisager tous les cas.
\paragraph{Itération}
On doit considérer trois formes d'itération : jusqu'à un échec, jusqu'à un point
fixe, et jusqu'à un échec ou un point fixe. Elles n'offrent toutes trois aucune
garantie de terminaison. On les note ici, respectivement \texttt{Rfail},
\texttt{Rid} et \texttt{RfailOrId}. On peut en définir deux commme suit~:
\begin{eqnarray}
\texttt{Rfail}(s) & = & \mu x. \; \texttt{Comp}([s,x]) \label{rfail:def:eq} \\
\texttt{Rid}(s)   & = & \mu x. \; ?)  \label{rid:def:eq} \\ 
\texttt{RfailOrId}(s) & =
     & \mu x. \; \texttt{Comp}([\texttt{IdentityAsFail}(s),x])
        \label{rfailorid:def:eq}
\end{eqnarray}


Comment définir $\texttt{Rid}(s)$ ? Ce problème suggère que notre ensemble
de transformations élémentaires n'est peut-être pas parfaitement bien choisi.

\paragraph{Contextuel}
Expliquer que, sans InnerContext, les règles de Green bouclent (donner un
exemple). J'ai déjà ajouté que, grâce à cette stratégie, on en réalise un grand
nombre sans boucler, mais cela n'apparaît plus.

\subsubsection{Fait}
AG : Modification du 2e paragraphe, car les transformations ne sont pas plus
générales que les stratégies, bonne remarque de WB.

\subsubsection{Remarques}
Le comportement de \texttt{TopDown(s)(t)} dépend du succès de l'application de
la transformation/stratégie \texttt{s} sur le terme \texttt{t}. Il y a deux
manières de détecter ce succès : (1) cette application n'a pas levé d'exception,
ou (2) cette application a produit un terme différent de \texttt{t}. Le critère
(1) est plus précis mais trop difficile à implanter en Maple. On retient le
critère (2), moins précis, car une application peut aussi
produire le même terme, mais suffisant en pratique.
Pour l'instant, seuls le top rewriting et le left choice (TODO) peuvent lever
une exception. Pour le top rewriting c'est le cas ssi la stratégie est une règle
(resp. conditionnelle) et que le matching n'a pas de solution (resp. qui
satisfait la condition). Voir tests dans la procédure test3() de regtest.mpl.
Comme All, par exemple, ne lève jamais d'exception, un TopDown(All(r))(t)
n'applique All(r) qu'à t, pas aux sous-termes de t (donc n'applique r
qu'aux sous-termes directs de t), ce qui n'est pas l'effet attendu. Pour obtenir
une approximation de cet effet, il faut écrire
TopDown(IdentityAsFail(All(r)))(t).
\begin{displaymath}
\begin{array}{|c l|}
\hline
 \texttt{All(s)(t)} =_{\textit{def}} & \texttt{if t=t'(t$_1$,$\cdots$,t$_n$) then}\\
    & \hspace{0.4cm}\texttt{t'(FailAsIdentity(s)(t$_1$),$\cdots$,FailAsIdentity(s)(t$_n$))} \\
    & \texttt{else         // t is a constant or a variable} \\
    & \hspace{0.4cm} \texttt{t;} \\
 \hline
\end{array}
\end{displaymath}


Pour TopDown, dans la définition l'effet nul de TopDown sur les constantes est
faux.
\begin{displaymath}
\begin{array}{|c l|}
\hline
 \texttt{TopDown(s)(t)} =_{\textit{def}} & \texttt{if  t=f(t$_1$,$\cdots$,t$_n$) then} \\
                          & \hspace{0.4cm} \texttt{try s(t);} \\
                               & \hspace{0.4cm}
                         \texttt{catch "Fail": f(\texttt{TopDown}(s)(t$_1$),$\cdots$,\texttt{TopDown}(s)(t$_n$));} \\
                        & \texttt{else // t is a variable or a constant} \\
                      & \hspace{0.4cm} \texttt{ FailAsIdentity(s)(t);} \\
\hline
\end{array}
\end{displaymath}

\paragraph{Comparaison avec Tom}
A droite d'une règle Tom, on peut mettre n'importe quelle expression Java,
avec un échappement pour construire un terme.

A droite d'une règle \ST, on écrit : ``the right-hand side of the rewrite rules
may contain calls of Maple$^{\mathsf{TM}}$ predefined functions or of functions
defined by the user. '', mais on devrait pouvoir généraliser à n'importe quelle
expression Maple.

\subsubsection{Réponse aux commentaires de ML}
``raising an exception'' is a standard notion in programming.


Les exemples pris dans cette partie sont nécessairement et volontairement donnés
sans référence à leur position dans la preuve, pour rendre cette partie
indépendante de la preuve (pas encore présentée) et pour éviter la critique
d'un langage conçu pour une seule preuve.
 
\subsubsection{Discussions}
What ARE transformations?  Essai de réponse en début de partie. A part le
``Expand'' de Maple, toutes les transformations utilisées dans la preuve du
gradient peuvent être considérées comme des stratégies. De plus, le
``Expand'' de Maple lui-même peut être remplacé par quelques règles de
réécriture. Par conséquent, proposer dans cet article une notion de
transformation plus générale que celle de stratégie est discutable. Faut-il
remplacer partout ``transformation(s)'' par ``strategy(ies)'' ?


Les stratégies \texttt{Identity} et \texttt{Fail} n'ont pas d'intérêt pratique
mais un intérêt théorique, que le degré d'avancement actuel du travail ne permet
pas encore de montrer. Faut-il en faire plus pour les justifier ?

La distinction expression/terme aide à clarifier un peu les choses, mais n'est
pas totalement satisfaisante.

C'est dommage que l'exemple de $t$ pour le InnerContext ne se retrouve pas
clairement dans l'annexe A.

\subsubsection{Removed sentences}
Strategies (and rules as basic strategies) apply to
expressions of a given formal language and transform them into other expressions
in the same language. In the model-driven engineering community they would be
called ``endogeneous transformations''. 

Now we show how to apply a transformation at some positions inside the term.

The syntax of terms is:
\begin{align*}
t ::= X\_ \;|\; f \;|\; f(t,\cdots,t) \; | \; f\_ (t,\cdots,t)
\end{align*}
where $f$ denotes a function name, $X\_$  a variable name,
 and $f\_$ denotes a variable function name i.e. a function of arbitrary name.
 For instance $var1_, f(var\_1,a), f\_(a)+sin(a)$ are terms.

The main programming concepts of our transformation language are the notions of
\emph{rules, strategies}, and \emph{transformations}. We mean by a rule a basic
rewrite rule. Strategies specify the way rules are applied and make it possible
to control the reductions. We provide a set of useful and the most often used
strategies as well as strategy constructors or combinators. The user can define
his own strategies by defining new Maple functions and eventually combining
already defined strategies.

Transformations  are (implemented as) Maple functions  possibly raising two
exceptions \ldots [[ TODO: define these exceptions and explain their meaning. ]]

Its semantics is given in form of an \emph{effective} rule.

It happened that a rule  might be
applied (namely with the \texttt{TopDown} transformation) to different subterms of a
given expression. However, we would like to apply it to just one of them

The point behind the application of the Green rule just to  \texttt{t$_2$}  is to
achieve a sort of normal form where the term $v$
 (also called the \emph{test function}, see Section \ref{}) is no longer under
 a $div$ operator.

Now we want to apply the rule  \texttt{ApproximationTSInv1}:
$\rrule{B(w\_)}{T^*w+O(\varepsilon)}$  to  $t_1$. And we want to apply the rule
\texttt{ApproximationTSInv2}: $\rrule{B(w\_)}{T^*(w)+ \varepsilon y.T^*(\nabla_x
w) +\varepsilon O(\varepsilon)}$  to $t_2$. The point
behind the
 application of  the rule \texttt{ApproximationTSInv2} to $t_2$ and not to $t_1$
is the presence of the $\frac{1}{\varepsilon}$ factor  which allows
simplifications.

With this constructor and the rule \texttt{multContext} previously defined as
above the rule

is to define a context-changing rule \texttt{context} by
$\rrule{X_}{\frac{1}{\varepsilon}XY\_}$. Therefore  \texttt{r\_epsilon} is the
rule 

\subsubsection{Suites}
A faire après soumission. Ajouter l'exception ``Interrupted'' dans le package,
la présenter ``Interrupted'' ici ou plus loin dans le texte. 
La commenter en lien avec
``STNormalizer''. Expliquer comment éviter la non-terminaison de ``Normalizer''
et limitant le temps de réécriture.

\subsection{Advanced features}

\subsection{Formal proof examples}

Le système proposé dans la partie 5.2 pour les $O()$ est plus simple
que le système réel écrit dans GradientProof/convergence.mpl.

\subsubsection{Fait}
Suppression du copyright dans les fichiers de règles (annexe E) (le copyright
sera dans l'archive soumise avec l'article) car cela rendait l'article trop
long. 

\subsubsection{TODO}
Enlever

\begin{verbatim}
#Recall that:
multContext := [X_,X*(1/Epsilon*Y_)];
\end{verbatim}

dans gradient*.*


Enlevé de twoscale.mpl :

\begin{verbatim}
#,
#               [B(X_*Y_), X*B(Y), DelayEval -> (VariablesSet(X)=[] ) ],
#               [B(X_), X, DelayEval -> (VariablesSet(X)=[] ) ]
\end{verbatim}

Revoir la description de l'annexe E. Pour l'intant, la partie ``Mathematical
operators'' n'en présente qu'une partie, dans le désordre, donc elle est
masquée.
La sous-preuve ``$u^0$ independent of $y$  proof'' n'étant pas expliquée dans 
cette partie, peut-on la cacner dans l'annexe.

convergence.mpl, gradient.mpl, hypothseis.mpl, integral.mpl
et twoscale.mpl utilisent OutermostNF qui n'est expliqué dans aucun fichier
LaTeX.

Les axiomes (\ref{O2}) and (\ref{O3}) et les règles de la partie 5.2 ne
correspondent pas parfaitement.


Move the linearity function from stmodule.mpl to
linearity.mpl. Ajouter la règle de sortie du scalaire, par une fonction paramétrée par ce
scalaire.

\subsubsection{Convergence calculus}
\paragraph{TODO}
Il y a deux sortes de convergences (weak et strong) et on n'utilise qu'une
seule notation $O()$. A clarifier.

Expliquer pourquoi la solution $\OEpsi{i}$ est naturelle.

Le système de règles proposé est-il assez riche ?

Signaler le problème des constantes.

Prouver que le système de règles est fortement normalisant. Les arguments
sont : Chaque règle fait décroître strictement la taille des expressions
auxquelles elle s'applique, donc toute séquence de réécritures est finie.
L'argument actuellement rédigé est insuffisant.

Choisir entre ``:'' et ``:='' pour donner un nom à une règle mais ne pas
utiliser les deux.

Mettre le code en police \texttt{texttt} au lieu de maths.

\paragraph{Discussions}
J'ai enlevé ``For any computed expression containing the two terms $\OEpsi{i}$
and $\OEpsi{j}$ this implementation guarantees that $i \neq j$.'', ``the fresh
index will never occur in any other term $\OEpsi{\ldots}$'' et la
\begin{proposition}\label{Fresh:Index:Prop}
Let $\mathcal{T}=\mathcal{R} \cup \mathcal{S}$, where $\mathcal{T,R,S}$
 denotes, respectively, a set of transformations, rewrite rules and strategy terms,
 where $\mathcal{R}$ contains $O(\varepsilon)$-rules.
 Assume that  $\mathcal{R}$ fulfills the requirement (REQ 1), and $\mathcal{S}$ fulfills
the requirement (REQ 2).
Let  $t$ be a term  and $s \in \mathcal{T}$ be a  transformation.
If $s(t)$ contains two terms $\OEpsi{i}$ and  $\OEpsi{j}$ then $i\neq j$.
\end{proposition}
 qui sont faux quand, par exemple, on développe $(a + b) * \OEpsi{i}$. 
Que faut-il prouver ?

\paragraph{Removed sentences}
 hence the function $FreshIndex()$
is evaluated at the \emph{declaration} of the rewrite rule.

a new index $i$ is chosen at each production of a term $\OEpsi{i}$.


One can prove that the convergence rewrite system above is 
terminating and confluent. This justifies  the use of the transformation
\texttt{ConvergenceStrategy} among other possible ones, consequently
  \texttt{ConvergenceStrategy} is also terminating.
 
To prove the termination it is sufficient 
to notice the application of each rewrite rule to a given expression strictly
 decreases its size. Therefore each rewrite sequence is finite.
  To prove confluence, it is sufficient
 to prove  that it locally confluent, see Newman's Lemma \cite{;} which states
 that a if a rewrite system  is terminating and locally confluent then it is
confluent.


\subsubsection{Linearity}


\subsubsection{Removed sentences}
``It is easy to prove that the convergence rewrite system  is terminating. It
is sufficient to notice that any application of a rewrite rule to a given
expression produces an expression with a smaller number of symbols. Therefore
each rewriting sequence with this system is finite. As shown in
Section~\ref{convergence:rules:sec} in Appendix~\ref{appendix:rules} we group
these rules with the \texttt{STNormalizer} and \texttt{LeftChoice}
combinators. The resulting transformation \texttt{ConvergenceStrategy} is
thus also terminating. 
We emphasize that the condition  ``if  $\alpha$
is independent of $\varepsilon$'' of the rule 
$\rrule{\alpha *O(\varepsilon)}{O(\varepsilon)}$  imposes an additional constraint 
on the \emph{type} of the term $\alpha$ so that the rewrite rule can be applied. 
Types are not considered in this paper. The integration of an
appropriate type system requires a separate work. 

The  convergence calculus given by the axioms (\ref{O2}) and (\ref{O3}) is turned
into a strongly normalizing rewrite system by orienting the equalities 
from the left to the right. This system will  be systematically used to
reduce expressions at each proof step.''


Appendices~\ref{appendix:gradient:math:proof}
and~\ref{appendix:gradient:maple:proof} prove of a part of
Proposition~\ref{gradient:approx:prop}.
\subsubsection{Done}
Explanation added about the second proof and how it uses the first one.
\subsection{Theoretical basis and related work}

\subsubsection{Tom}

\subsubsection{Elan} 
In  \cite{RewriteStrat_CHK2003} it was showed   that the strategies might be
expressed with  the $\rho$-calculus itself. In other words the strategies may be
viewed as higher order rewriting rules. In the \ST language the strategies are expressed
by means of higher order functions thanks to the fact that our host language
Mapple support functional programming. The idea of considering term  rewriting  from a
functional point of view was done  in \cite{BKK+99}.
\mycomment{WB}{Same problem mentioned above, failure as the empty set. }

\subsubsection{Removed sentences}
The idea of the $\rho$-calculus  is to integrate in a uniform way the matching, the
rewriting and non-determinism.

\begin{itemize}
\item Putting forward the use of the strategy language for the automatisation 
 of  the two scale transformation.
\item The implementation of the \ST language can be done easily? yes, can
be done within any functional programming language.
\end{itemize}

``is one of the
characteristics of the $\rho$-calculus, and it might''

\subsection{Acknowledgements}
Added. Remerciements à Bin et Raj pour avoir utilisé le package.

\subsection{Conclusion}
\subsubsection{Fait}
``Maple'' remplacé partout par Maple$^{\mathsf{TM}}$.

\subsubsection{TODO}
Il faut conclure sur la manière dont on a levé les critiques sur la réécritue
dans Maple. 

\subsubsection{Extra sentences}
A intégrer ?

``This requires that the types of the initial terms has to be specified and then
 propagated to the resulting terms during the transformation process.''
 
 
\mycomment{WB}{One of the problems is that  the transformations contain both
controllable rewrite rules and uncontrollable computations. The latter are
performed by the host language Maple.} 


Moreover, this  work brings an insight to more ambitious objectives which can be
regrouped in two categories, namely generalization and automation. The
generalization objective consists in the construction of a unique \emph{proof
algorithm} for many other convergence proofs than the gradient ones.  The
automation objective consists in minimizing the human intervention by performing
automatically a long sequence
  of transformations.

\subsection{References}
\cite{BBK_Tom07} pas assez précis.


\subsection{Appendix A}
\subsubsection{Fait}
Ajouts de retours à la ligne pour les formules trop larges dans les steps 6 et
9.

\subsubsection{Remarques}
J'ai déplacé la position du step 7 dans la preuve mathématique pour qu'il
coïncide avec le step 7 de la preuve formelle.
 
\textbf{Step 7.} We use Assumptions $Tu=u^{0}+O(\varepsilon )$ and $%
Tu=u^{0}+\varepsilon u^{1}+\varepsilon y.\nabla _{x}u^{0}+\varepsilon
O(\varepsilon )$ in the first and in the second integrals respectively%
\begin{align*}
\Psi =& -\int_{\Omega \times Y}(u^{0}+O(\varepsilon ))\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y}\big(u^{0}+\varepsilon u^{1}+\varepsilon y.\nabla
_{x}u^{0}+\varepsilon O(\varepsilon )\big)\;\big(\frac{1}{\varepsilon }%
\;div_{y}v+y.\nabla _{x}div_{y}v\big)\text{ }dxdy+O(\varepsilon ).
\end{align*}%
Expanding the parentheses and simplifying the vanishing terms,%
\begin{align*}
\Psi =& -\int_{\Omega \times Y}u^{0}\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y}(\frac{1}{\varepsilon }u^{0}+u^{1}+y.\nabla
_{x}u^{0})div_{y}v\;dxdy \\
& -\int_{\Omega \times Y}u^{0}y.\nabla _{x}div_{y}v\;dxdy+O(\varepsilon ).
\end{align*}%
% \begin{equation*}
% \Psi =-\int_{\Omega \times Y}u^{0}\;div_{x}vdxdy-\int_{\Omega \times Y}(%
% \frac{1}{\varepsilon }u^{0}+u^{1}+y.\nabla _{x}u^{0})div_{y}v\text{ }%
% dxdy-\int_{\Omega \times Y}u^{0}y.\nabla _{x}div_{y}v\text{ }%
% dxdy+O(\varepsilon ).
% \end{equation*}


[[ Alain: autre preuve. On développe : ]]

\begin{equation*}
\Psi =-\int_{\Omega \times Y}Tu\;div_{x}v\,dxdy-\int_{\Omega \times Y}Tu\;
\frac{1}{\varepsilon }div_{y}v dxdy -\int_{\Omega \times Y}Tu\;y.\nabla
_{x}div_{y}v dxdy+O(\varepsilon ).
\end{equation*}

We use Assumptions $Tu=u^{0}+O(\varepsilon )$ and $%
Tu=u^{0}+\varepsilon u^{1}+\varepsilon y.\nabla _{x}u^{0}+\varepsilon
O(\varepsilon )$ respectively in the first and third integrals and in the second
integral%
\begin{align*}
\Psi =& -\int_{\Omega \times Y}(u^{0}+O(\varepsilon ))\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y}\big(u^{0}+\varepsilon u^{1}+\varepsilon y.\nabla
_{x}u^{0}+\varepsilon O(\varepsilon )\big)\;\frac{1}{\varepsilon }%
\;div_{y}v \;dxdy \\
& -\int_{\Omega \times Y} (u^{0}+O(\varepsilon ))\;y.\nabla _{x}div_{y}v\;dxdy+O(\varepsilon ). \end{align*}%

After simplification

\begin{align*}
\Psi = & -\int_{\Omega \times Y}u^{0}\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y}(\frac{1}{\varepsilon }u^{0}+u^{1}+y.\nabla_{x}u^{0})div_{y}v\; dxdy \\
& -\int_{\Omega \times Y}u^{0}y.\nabla _{x}div_{y}v\; dxdy+O(\varepsilon).
\end{align*}

[[ Fin autre preuve. On retombe sur la suite du step 7, mais le choix de
l'ordre d'approximation, guidé par la présence de $\dfrac{1}{\varepsilon}$ est
plus facile à faire par OuterContext. Michel, es-tu d'accord ? ]]

[[Michel: Tu peux faire la démonstration comme tu la veux, mais il faut
qu'elle soit robuste. Bref, si cela t'arrange d'avoir le $1/\varepsilon $ à
un certain endroit, il faudrait pouvoir l'y amener automatiquement. Car à un
moment de preuve, on peut tout à fait avoir ce terme à un autre endroit. Il
faut certainement raisonner modulo des formules équivalentes, et si né%
cessaire travailler sur une forme "canonique" qui arrange. Si nous n'avons
pas cette exigence aujourd'hui, nous ne pourrons pas aller très loin.]]

Remplacement de
\begin{align*}
\Psi =& -\int_{\Omega \times Y}u^{0}\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y}(\frac{1}{\varepsilon }u^{0}+u^{1}+y.\nabla
_{x}u^{0})div_{y}v\;dxdy \\
& -\int_{\Omega \times Y}u^{0}y.\nabla _{x}div_{y}v\;dxdy+O(\varepsilon ).
\end{align*}
par une forme normale totalement développée, seule accessbile par calcul

\begin{align*}
\Psi =& -\int_{\Omega \times Y}u^{0}\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y} \frac{1}{\varepsilon }u^{0} div_{y}v\;dxdy \\
& -\int_{\Omega \times Y} u^{1} div_{y}v\;dxdy \\
& -\int_{\Omega \times Y} y.\nabla_{x}u^{0} div_{y}v\;dxdy \\
& -\int_{\Omega \times Y}u^{0}y.\nabla _{x}div_{y}v\;dxdy+O(\varepsilon ).
\end{align*}

\textbf{Step 7. }

[[Walid : dans la preuve formelle, toutes les applications successives de la
formule de Green se font en une seule stratégie. Donc, ce serait mieux de
mettre le calcul suivant en début de step 8, plutôt qu'en fin de step 7.
C'est plus facilement automatisable si on développe davantage. ]]

[[ Alain : par exemple, pour pouvoir dire précisément où on applique la
formule de Green suivante, il faut écrire l'expression précédente comme suit
: ]]

[[Michel: vous appliquez les formules de Green là où vous voulez...]]

\begin{align*}
\Psi =& -\int_{\Omega \times Y}u^{0}\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y}\frac{1}{\varepsilon }u^{0}div_{y}v\;dxdy \\
& -\int_{\Omega \times Y}(u^{1}+y.\nabla _{x}u^{0})div_{y}v\;dxdy \\
& -\int_{\Omega \times Y}u^{0}y.\nabla _{x}div_{y}v\;dxdy+O(\varepsilon ).
\end{align*}

Applying the Green formula
\begin{equation*}
\int_{\Omega \times Y}u^{0}div_{y}vdxdy=\int_{\Omega \times \partial
Y}u^{0}v.n_{Y}dxds(y)-\int_{\Omega \times Y}\nabla _{y}u^{0}.vdxdy,
\end{equation*}%
where $n_{Y}$ stands for the unit outward normal vector to the boundary $%
\partial Y$ of $Y,$ and remarking that $\nabla _{y}u^{0}$ vanishes, and that
$v$ vanishes on $\partial Y$, it remains%
% \begin{equation*}
% \Psi =-\int_{\Omega \times Y}u^{0}div_{x}v\;dxdy-\int_{\Omega \times
% Y}(u^{1}+y.\nabla _{x}u^{0})div_{y}v\;dxdy-\int_{\Omega \times
% Y}u^{0}y.\nabla _{x}div_{y}v\text{ }dxdy+O(\varepsilon ).
% \end{equation*}
\begin{align*}
\Psi =& -\int_{\Omega \times Y}u^{0}\;div_{x}v\;dxdy \\
& -\int_{\Omega \times Y}(u^{1}+y.\nabla _{x}u^{0})div_{y}v\;dxdy \\
& -\int_{\Omega \times Y}u^{0}y.\nabla _{x}div_{y}v\;dxdy+O(\varepsilon ).
\end{align*}

\subsection{Appendix B}

\subsection{Appendices C et D}
Code parfois trop large, réduit en small.

Preuve formelle de ``$u^0$ is independent of $y$'' cachée, pas le temps de la
vérifier. C'est un lemme. Dit dans encoding.tex.

\subsection{Appendix E}
There was an error at Step 6 in GradientProof/heat.mpl SVN 2685. It produced

\begin{verbatim}
BigO(24,Epsilon)+SUM(
 Integral([TSTM(Omega),TSTm(Omega)],
  (partial(v0,x(i))+partial(v1,y(i)))*a0*T(partial(u,x(i))),[x, y])
 +BigO(22,Epsilon),
 i,Iset)
 -Integral([TSTM(Omega), TSTm(Omega)],v0*f0,[x, y])
\end{verbatim}

instead of 

\begin{verbatim}
BigO(28,Epsilon)+
 SUM(Integral([TSTM(Omega), TSTm(Omega)],
  a0*(partial(u0,x(i))+partial(u1,y(i)))*(partial(v0,x(i))+partial(v1,y(i))),[x, y]),i,Iset)
 -Integral([TSTM(Omega), TSTm(Omega)],v0*f0,[x, y])
]
\end{verbatim}

Il manquait une étape 
\begin{verbatim}
EqTerm := Outermost(LinearityOf[SUM])(EqTerm);
\end{verbatim}
pour isoler le $O()$. C'est corrigé.

Les règles paramétrées sont dangereuses. Ajouter un commentaire sur les
conditions d'utilisation. Augmenter la paramétrisation ($j, J$).

\subsubsection{Code cleaning}
Removed:

\begin{verbatim}
# From convergence.mpl:

#OEpsilonSumContext:=OuterContext(OEpsilonSum)([X_,Z_+X]);

# OEpsilonSUMContext:=
#   OuterContext(OEpsilonSUM)([X_, SUM(Y_+X,J_,D_)]);
\end{verbatim}

\subsubsection{TODO}
Dans integral.mpl, le remplacement de

\verb!Linearity2Of[partial] := [partial(Epsilon*F_,X_),Epsilon*partial(F,X)];!

par 

\verb!Linearity2Of[partial] := Linearity2(1,partial(X_,Y_),Epsilon );!

n'a pas été documenté.

\subsection{Appendix F}
Caché.


\subsection{Discussion}
\subsubsection{Décembre 2013}
ML : je ne suis pas satisfait par les définitions de substitution, matching et
règle de réécriture. Lors de la rédaction, je ne m'étais pas plongé dans ce
domaine et je ne pouvais pas me prononcer dessus. A présent, j'ai l'impression
d'y voir plus clair (peut-être que je me trompe) et en l'état je trouve que ces
définitions ne sont pas très bien formulées. Mais comme ce n'est pas moi qui les
ai écrite, je trouve qu'il est inadapté que je les change. Qu'en penses-tu?

AG : Ces définitions sont écrites de manière très standard. Tu peux par exemple
comparer avec le contenu des pages 20 et 64 du document joint, qui fait
référence dans ce domaine. Je ne vois pas ce qui pourrait ne pas convenir.

Si tu as une idée d'autre formulation, tu peux m'en l'envoyer séparément. Je
l'examinerai et comprendrai peut être ce qui te gène.

\subsubsection{Juillet 2011}

AG : La preuve de l'équation de diffusion est rédigée comme un calcul formel qui
aide le mathématicien à obtenir la bonne définition de $a^H$ et de $f^H$. Ce
genre de preuve est en général composée d'une phase d'expansion, suivie d'une
phase de contraction, dans lesquelles les mêmes règles sont utilisées en sens
inverse. On ne peut donc pas automatiser ces calculs sans risque de non
terminaison. La preuve du gradient aurait pu être présentée de la même manière.
Les étapes 1 à 6 de la preuve de l'équation de diffusion utilisent la ``théorie
multiscale'' (renvoi à l'annexe E). On intuite que cette phase est plus
facilement généralisable que les étapes 7 et suivantes, qui nécessitent une
expertise mathématique et l'ajout de règles spécifiques. C'est pour cela qu'on
n'a pas formalisé la fin de la preuve mathématique.

\subsubsection{Pattern-matching}
[[ Alain: optional section. ]]

[[ Alain : what about \texttt{::indefinite}? Walid: This is also a type. The
point is that declaring a variable via its type is not natural. ]]

Maple provide us with the function \texttt{patmatch(expr,pattern)} for
pattern-matching. The main drawback of \texttt{patmatch} is that the user has to
declare the variables by specifying their types, e.g.
\texttt{patmatch(x+3,a::name + b::integer)}.
Moreover \texttt{patmatch} returns just one (possibly empty) substitution. Hence
this function is not useful if one needs to compute many substitutions, in
particular, if the computations are not deterministic. In this case the user has
to define his own matching function.



It is worth mentioning that matching modulo a theory is related to
non-determinism, in the following sense. When computable, the matching process
can return zero, one or many results (i.e. substitutions), possibly infinitely many. Therefore,
for each result, the application
 of a rewrite rule to a  term can yield zero, one, or many (possibly infinitely
 many) terms. On the one hand, we expect 
 mathematical proofs to be deterministic. On the other hand, dealing with
  non-determinism requires
an extra set of strategies and constructors which make the language unnecessary
complicated in practice. For these reasons the \ST language is restricted
to the deterministic fragment. Matching modulo AC is minimally implemented
by returning at most one solution, but always the same one. One future work is
to address this issue in a way adapted to mathematician needs. 

%\subsubsection{The \ST language as a fragment of the  $\rho$-calculus}
 
\subsubsection{A propos du langage de transformation}

 - Justification of extensability to non-deterministic strategies, matching
 modulo AC and more, proof search, proof objects (as in rhoLog), user-defined
 strategies.

Le langage de transformations proposé dans la partie 3 a permis (en décembre
2010) d'écrire une preuve formelle de la propriété de convergence du gradient au
même niveau que la preuve mathématique qu'elle formalise. Cette notion de
``niveau'' de démonstration recouvre plusieurs aspects : (1) Les deux preuves
sont de longueurs comparables, (2) les deux preuves suivent les mêmes étapes de
raisonnement (voir plus loin à ce sujet la notion d'algorithme de démonstration)
et (3) la stratégie à écrire à chaque étape de la preuve formelle est une
formalisation naturelle (simple et quasi-systématique) de la phrase explicative
rédigée dans la preuve mathématique. 

Cette formalisation à niveau égal atteint un premier objectif, qui est de
fournir au mathématicien un langage pour formaliser aisément ses raisonnements
équationnels (et d'approximation). Le langage proposé a rendu le coût de
formalisation très inférieur à ses bénéfices immédiats, qui sont multiples [[ Il
faudrait plus d'expérimentations pour étayer cette affirmation.]]. Le bénéfice
principal est une forte garantie de correction de tous les calculs
intermédiaires. S'y ajoutent les possibilités d'explorer rapidement des
variantes de la démonstration, de combiner directement ces raisonnements avec
tous les calculs algébriques usuels, et de produire rapidement et avec
fiabilité, car mécaniquement, un texte de démonstration aussi précis que celui
qui aurait été laborieusement composé sans ces outils. Tous ces nouveaux moyens
se traduisent globalement par un considérable gain de temps. 

Quoique modeste, ce premier objectif était donc loin d'être négligeable.
D'autant plus qu'il ouvre la porte à des objectifs plus ambitieux qu'on peut
regrouper dans 3 catégories, qui sont la généralisation, l'automatisation, et le
contrôle du niveau de détail. 


La généralisation est associée à la notion d'algorithme de démonstration. Par
expérience, on sait déjà que les mêmes étapes que celles de la preuve du
gradient conviennent pour beaucoup d'autres preuves similaires (voir notes de la
réunion du 30/11/2010). C'est ce qu'on appelle l'\emph{algorithme de
démonstration}. La généralisation consiste à construire cet algorithme unique
qui enchaîne tous les calculs d'approximation requis dans de nombreuses
situations. On procédera par généralisations progressives. 


Dans la direction de l'automatisation, l'objectif est de réduire l'effort
d'intervention du mathématicien en enchaînant automatiquement et implicitement
de longues séquences de calculs (comme Maple le fait déjà sur l'aspect
algébrique des expressions). C'est une problématique classique en démonstration
formelle. On appliquera des méthodes usuelles dans ce domaine pour établir que
certains systèmes de réécriture terminent et sont (éventuellement) confluents.
Ces techniques ont déjà été appliquées dans le présent travail, où l'on a
montré, à titre d'exemple, que le système de convergence était terminant et
confluent (aux indices des $\OEpsi{\ldots}$ près). Ces propriétés ont permis
d'appliquer systématiquement ce système entre chaque étape de preuve, allégeant
d'autant le travail de formalisation de la preuve. Comme on sait déjà que
l'union de toutes les règles de réécriture utiles n'est pas un système
terminant, cette tâche d'identification doit être faite soigneusement sur de
nombreux sous-systèmes. Elle peut être considérablement facilitée par
l'identification préalable de tels sous-systèmes candidats. Cette identification
peut être faite par le mathématicien, car les bons et les mauvais candidats ont
en général une signification mathématique. Néanmoins, comme cette approche
analytique restera toujours laborieuse et partielle, on la complètera par une
approche expérimentale, empirique mais facile à mettre en oeuvre (on interrompt
une recherche automatique jugée trop longue).  

L'inconvénient majeur de l'automatisation est bien connu. C'est la perte de
contrôle sur le cheminement de la preuve. Trop d'automatisation génère des
expressions trop complexes pour que le mathématicien puisse les analyser
efficacement et suggérer une étape suivante pertinente. Ce problème peut être
considérablement réduit en combinant les ingrédients suivants. Le premier, déjà
mentionné, est de regrouper en systèmes des règles de calcul ``de la même
famille'', de nommer ces systèmes, et de faire générer par le prouveur automatique
une trace des étapes qu'il a suivies, en indiquant quels systèmes il a appliqué,
et selon quelle stratégie. Un langage de haut niveau pour ces traces a été
proposé dans ce document. Un deuxième ingrédient, lié au premier, est d'offrir
la possibilité de contrôler le niveau de détail des preuves produites. Cela
s'inscrit dans la 3e catégorie d'objectifs. A ce jour, la nature exacte de ce
mécanisme de zoom avant et arrière sur les preuves n'est pas encore totalement
établie. Un troisième ingrédient sera la possibilité de guider la preuve
automatique dans une direction plutôt qu'une autre. Dans ce domaine, les moyens
sont nombreux. On peut contrôler le nombre et la nature des enchaînements de
transformations, spécifier la forme de la cible, etc.


Une première étape dans la direction de ces objectifs sera une expérimentation de
``raccourcissement de la preuve'', progressive. Pour cette
expérimentation, on propose les étapes suivantes :

1. Modulo convergence. Chaque étape de la preuve actuelle se termine 
par

LHSterm := ConvergenceStrategy(LHSterm);

sans risque, puisque cette stratégie est terminante et confluente.

Supposons que l'étape soit, par exemple 

LHSterm:=TopDown((Transform(LazyEval(ApproximationT[1]))))(LHSterm);

On combinera le tout en encapsulant dans une
transformation de plus haut niveau la sequence suivante :

LHSterm := Transform(
 Comp(
  [
   TopDown((Transform(LazyEval(ApproximationT[1])))),
   ConvergenceStrategy
  ]
 )(LHSterm);

2. Additionally modulo integral calculus.

LHSterm := Transform(
 Comp(
  [
   TopDown((Transform(LazyEval(ApproximationT[1])))),
   ConvergenceStrategy,
   IntegrationStrategy
  ]
 )(LHSterm);

 si on hiérarchise les stratégies, ou bien

LHSterm := Transform(
 Comp(
  [
    TopDown((Transform(LazyEval(ApproximationT[1])))),
    LeftChoice(
     [
      ConvergenceStrategy,
      IntegrationStrategy
     ]
    )
  ]
 )(LHSterm);

 si on met les deux stratégies en parallèle.

 
 Continuer ainsi et observer à chaque étape si :
 
 - La preuve termine toujours ?
 
 - C'est toujours la ``même'' preuve (en un sens à définir) ?
 
 - Le nombre d'étapes diminue ?
 
 - On comprend encore ce que fait la machine ?
  
Remarquer que, dans le terme de stratégie ainsi construit, il y a des
``inconnues'' qui sont les choix dans les LeftChoice, les positions des TopDown,
le nombre d'itérations dans les Normalizer. Il y a donc deux sortes d'objets
de preuve : le ``proof guide'', qui est ce terme de stratégie qui sert à guider
un prouveur automatique, et le ``proof trace'' qui est la preuve effectivement
prouvée, plus précise (définir cette inclusion). 
Le proof guide est une contrainte, une sûreté. Il faut ajouter un objectif,
une vivacité, un pattern à atteindre. Par exemple ``Normalizer'' fixe la contrainte
de normalité du résultat (non transformable).

Distinguer stratégies de sûreté et de vivacité ? 


\subsubsection{Justifier l'exclusion du non-déterminisme}
 
 Comment justifier l'absence de non-déterminisme dans le langage de
 transformations proposé ? Here we provide a language de proof traces and a
 proof trace animator. It avoids many human errors. It organizes axioms in theories. It is a first milestone, extensible.
L'indéterminisme serait dans un langage de ``proof guides''. Proof traces are
normal forms of proof guides wrt some refinement relation to define inductively
and syntactically. A prover is a ``proof guide normalizer''. Other kind of work.
Too long to be treated here.
 
\subsection{Historique}
Dans l'ordre chronologique.

\subsubsection{Michel, 25/11}
Bonjour Alain, Concernant l'article en préparation, Je t'envoie ci-joint ma
contribution et qq remarques dans les fichiers. En fait, en continuant à lire, je
me suis rendu compte que j'ai beaucoup de remarques. Certaines sont des détails,
je n'en parle pas ici. Les autres sont trop nombreuses pour être données ici.
J'en fais juste quelques unes. Je trouve que le contenu de l'article est encore
un peu loin (de mon point de vue) d'être publiable.

D'une façon générale, je ne vois pas la relation qu'il y a entre les énoncés qui
se trouvent dans la section "2. Preliminaries and notations" et le programme à la
fin de l'article.

[\textbf{WB}: Now the program at the appendix is updated using the current version of the tool
 \texttt{symbtrans}]
Par exemple dans la définition d'une règle la condition de
transmission des variables d'une règle ne me semble pas satisfaite dans les
exemples.

[\textbf{WB}: It is written in a compact way in the section Preliminaries in terms of the
 matching and the substitution.]

A mon avis, le terme distributivité n'est pas utilisé dans son acception
habituelle en maths. Ici, il s'agit de linéarité. Je me demande, s'il ne serait
pas possible d'attribuer une propriété une fois pour toute à des « opérateurs »,
comme la propriété de linéarité, plutôt que de la définir pour chaque cas.


[\textbf{WB}: Done, see subsection \ref{linearity:sec} and some tests are
in the file \texttt{.../rewriting/RhoMaple/lambda.mpl}]
 Dans
les appendices il y a beaucoup à dire. Il faudrait se rencontrer. Je donne juste
quelques exemples.


Appendice A :

-    L'énoncé de la proposition 6 n'est pas très bien sous cette forme, il faut
en reparler directement.

-    Je propose de supprimer la notation "bar" mais remplacer par un opérateur
"B". [\textbf{WB:}Done.]

-    J'aurai plutôt mis des lemmes préliminaires (comme les règles sont établies
séparément).

-    Il faudrait définir la fonction v avec ses conditions au bords (=0).

-    L'étape 8 contient beaucoup d'erreurs.

-    Il faudrait formuler toutes les hypothèses faites depuis le début et ne pas
les rajouter au fur et à mesure.

Appendice C :

-    Je trouve que de nombreuses règles ne satisfont pas la règles de réécriture.

-    « AdjointDef » semble faire double emploi avec « TwoScaleAdjointInv »
 [\textbf{WB:}OK, \texttt{AdjointDef} rule deleted.]

-    « ApproximationTS » et « ApproximationTS2 » devraient être groupés dans une
même règle paramétrée. Idem pour les « ApproximationTSInv1 » et sa grande s?ur.
 [\textbf{WB:}Done.]

-    Je ne vois pas de O(epsilon) dans la règle « OEpsilon\_const » [\textbf{WB:}Corrected.]

 \subsubsection{Walid, 30/11}
\begin{itemize}
\item \texttt{OuterContext} strategy  was false. It is corrected now.
\item I add the Subsection \ref{linearity:sec} on the Linearity. The old distributivity rules
  in the Appendix are rewritten with the Linearity constructor.
\item \texttt{Normalizer} strategy is implemented and used instead of the old
 \texttt{NF} one.
\item Step 7 in the Gradient proof: a more complicated (+-)  OuterContextual
 rewriting  appears. I have integrated it instead of the old way of using the
 substitution. [[ Alain : preuve revue, OuterCOntext plus simple, voir avec
 Michel. ]]
\item I added the file \texttt{hypothesis.mpl}
\end{itemize}

 \subsubsection{Walid, 01/12}
\begin{itemize}
\item \texttt{bar} is replaced with \texttt{B}. Moreover, \texttt{TSTM} and
\texttt{TSTm} are used.

\item Step3 in the semi-automatic proof of the gradient uses the strategy
\texttt{OuterContext} to express
 the behaviour of $v$ and $B(v)$ on the Boundary, see \texttt{hypothesis.mpl}.

\item I added  the  table \texttt{LinearityOf}  that includes the set of linear
operators, namely \texttt{Integral} and \texttt{TwoScale}. To obtain the rewrite
rule that corresponds to the linearity of \texttt{Integral},
 we just write \texttt{LinearityOf[Integral]}.

\texttt{PS}. To declare an operator as Linear just use the function
\texttt{Linearity}, see the manual of \texttt{Linearity}, section
\ref{linearity:sec}.


\item The strategy combinators: \texttt{LeftChoice,Composition} are implemented
and tested dans RhoMaple/lambda.mpl.

\item A strategy  that allows to perform transformations/rewriting modulo the theory of
 $O(\varepsilon)$ is added, it is called \texttt{ConvergenceStrategy},
   see file \texttt{convergence.mpl}  or Appendix C, subsection convergence
   rules. It is tested in the file \texttt{Lambda.mpl}.

[[ Alain : Peut-on remplacer partout les règles sur Epsilon par la theorie ? ]]
\item The  rules \texttt{ApproximationTS,ApproximationTS2,...} are regrouped.
  It is possible to express them in a more compact way by means of
 just one  rule if  the approximation formula (at any order) is available.
\item The package now supports  the conditional rewriting rules.

 \textbf{Problem:} strict evaluation at the level of conditions when the
 conditional rule is declared.

 [[ Alain : question à étudier après l'article, hors sujet. ]]
\item I stopped at step7 at the semi-automatic proof.
\end{itemize}


 \subsubsection{Walid, 02/12}
\begin{itemize}
\item Gradient proof finished with a good level of generality:
 \begin{enumerate}
 \item The use of \texttt{ConvergeceTheory} strategy to compute "modulo?"
 convergence theory. Proof steps are dramaticaly reduced. The same thing can
 be done for the Integral calculus, but this would make the proof too compact.

 [[ Alain : do experiments. ]]
\item Green Rules regrouped into one using the strategy combinators. Another
solution is to use conditional rules(Impossible, see bellow).

\item The successive applications of Green rules until all the $v$'s  are out of
the $div$   are expressed by just one strategy.

[[ Alain: checked. ]]
\item Idem for vanishing terms on the boundary. [[ Alain: pour l'instant, on
fait suivre toute Green rule d'une boundary dans la preuve. Généraliser ? ]]
 \end{enumerate}
\item I am convinced that the general algorithm given by Michel at the last
meeting might be expressed by our  \emph{strategy language}. The idea is that
 the combinator strategies are a sort of \emph{temporal} operators.  Therefore,
 this strategy language corresponds to a (useful and powerful enough)
  fragment of the $\mu$-calculus.

 [[ Alain : et meme sans $\mu$-calculus, il s'agit de construire les bonnes
 stratégies. ]]
\item I modified and corrected some parts of the paper.
\item Conditional rules are \textbf{impossible} to implement correctly because
of two reasons:
\begin{enumerate}
\item strict evaluation of the conditions of the rules, and
\item undeterminism is \textbf{necessary}. (Technical arguments).
\end{enumerate}

[[ Alain : étude après article à faire, liée au typage. Plus besoin dans la
preuve du gradient. ]]
\end{itemize}

 \subsubsection{Walid, 03/12}
\begin{itemize}
\item I added the function \texttt{LazyEval(r)(t)}, that evaluates
 the $O(\varepsilon)$-rule \texttt{r},  i.e. applies the rule \texttt{eval}
 to \texttt{r}, see the file \texttt{GradientProof/LazyEval.mpl}.

 [[ Alain: warning: see restriction in LazyEval.mpl. ]]
  \item I did some  modifications and corrections on sections 3 and 4 of the paper.
 \end{itemize}

 \subsubsection{Walid, 04/12}
\begin{itemize}
\item The strategy \texttt{BottomUp} is implemented, and tested. Its explanation
 is written in the paper. Is an example that illustrates this strategy necessary?

 [[ Alain : yes. ]]
\item \texttt{normalizer,comp} are replaced with  \texttt{Normalizer,Comp}.
\item Section \ref{encoding:sec} revised.
\item \mycomment{AG}{\emph{Quel pourcentage de la preuve initiale se fait
actuellement automatiquement, en appelant seulement Normalizer sur le choix de
toutes les règles ?}}

\textbf{WB:}
Tout sauf les deux "run time rules", i.e. les regles  qui produisent
 la bonne approximation (au moment de l'execution )
 en fonction du degres de epsilon. i.e. les deux  OuterContext (Step5, 6).
Je dis ca car je fais semblant que je ne connais pas a priori le degre de
 epsilon.
Ce type de regles peut etre completement automatise' (cela va repondre a une
 question pose'e par Michel juste avant que tu rentre dans la salle,
 derniere reunion du 30/12) comme ca:\\
 A chaque fois qu'une regle d'approximation est applicable :
\begin{enumerate}
\item chercher le degre de epsilon,
\item produire le contexte correspondant
 \item produire la regle d'approximation contextuelle correspondante
   (ceci est necessaire si il y plusieurs sous termes, chacun avec un degres de epsilon
 different)
 \item appliquer la regle de l'etape 3.
\end{enumerate}

On peut exprimer  ces 4 etapes par une strategie, lui donner un nom, et
 l'integrer dans l'algo general.

 J'aime bien que certaines regles s'executent comme tache de fond, ex. les hypotheses.
Mais ca sera du sucre syntaxique.


\end{itemize}


\subsubsection{Walid et Alain, 06/12}
TODO, in decreasing order of priority:

- Pas compris Green.mpl : div et nabla.\mycomment{WB}{corrected}

- Préciser dans l'article la place exacte du LazyEval après production de O()
et la restriction.\mycomment{WB}{Corrected, and explained in the paper, see the Proposition
 \ref{Fresh:Index:Prop}}

- Réfléchir à la condition ``constante" dans convergence.mpl

- Stabiliser la preuve de gradient + sorties (largeur page, police).

- Experiment proof compaction, towards automation. For the paper.

- Discussion et conclusion :

- Excessive use of Transform(\ldots)?

- separate math lemmas and multiscale lemmas.

- Move Linearity from symbtrans.mpl to ???

- add LinearityOf[TwoScaleScalarMult] in twoscale.mpl.

- research: How to distinguish a scalar? (typing-like requirement, or
conditional rule).


\subsubsection{Walid, 7/12}
Révision preuve Maple selon consignes Michel.

-The scalar product is represented by a new operator \texttt{ScalProd(x,y)}, its properties are
 in the file \texttt{scalars.mpl}. We do not use maple scalar product operator because
 it imposes  that the operands are vectors.

- Green rules corrected according to the previous consideration. Michel mentioned
   another particular instance of the Green rule that applies to  $y.\nabla(...)$,
  last term of \texttt{Step 8}. It is added and
 the semi automatic proof becomes less generic (Updating the Mathematical proof?).


- The semi automatic proof as well as some hypothesis are
 redone using  the \texttt{ScalProd(x,y)} operator.

- Expressing the behavior of $v$ and $B(v)$ my means of the  \texttt{OueteContex} become
 ad hoc.

-Modif end Sec 4.
\subsubsection{Alain, 7/12}
Partie 3 revue. Preuve mathématique retouchée.
Attention : on accepte qu'elle diffère de la preuve formelle. A reprendre en
discussion.

Ce qui reste à résoudre :

Pour OuterContext, les problèmes liés à la convention d'underscore pour les
variables à gauche des règles et pas à droite,
\mycomment{WB}{C'est le $\rho$-calcul qui impose qu'on n'introduit pas de nouvelles variables a droite
 des regles, cela n'a rien a voir avec le underscore. Les regles de contexte sont une
exception, le combinateur \texttt{OuterContext}  a une semantique particluliere. (deja explique\'e dans le papier? )}

la nature des règles, la
condition des variables à droite toutes à gauche.

Indiquer assez tôt que le matching de la réécriture se fait modulo AC pour les
opérateurs + et * de Maple, avec choix de la première solution. Critiquer ce
choix mais dire que ce n'est pas le sujet.

En Maple on code le produit numérique et le produit scalaire par le même
symbole *. \mycomment{WB}{Dangeroux, car le matching se fait modulo AC pour
 *. J'ai introduit le produit scalar}

\subsubsection{Michel, 07/12}
Limites de la méthode rédigée, remarques.

Il faut une règle suivant laquelle chaque terme t peut être une
fonction de epsilon mais il doit avoir une limite t0 quand epsilon
tend vers 0. Cela exclu la possibilité qu'il y ait du 1/epsilon dans
un terme.

Il faut préciser les limites dues au fait que les variables ne sont pas typées :

-\qquad Dans la manipulation de vecteurs et de scalaires (ici v, la
normale extérieure n et nabla sont des vecteurs alors que u, div()
sont des
scalaires) les multiplications ne sont pas commutatives. Cela pose un problè%
me de fond par le fait que par ailleurs les opérations que nous
faisons sont définies modulo l'addition et la multiplication. Ceci
est une grosse source d'erreur dans les calculs.

-\qquad La définition de la linéarité par rapport à la
multiplication par une constante ne peut pas être faite dans un sens
général (on la définit seulement pour la multiplication par rapport
à 1/epsilon) puisqu'on ne distingue pas les fonctions des
constantes.

Concernant la gestion des noms de variables de fonctions:

-\qquad Les variables des fonctions ne sont pas écrite (cela devrait
être dit quelque part)

-\qquad Les variables sont précisées dans les mesures des intégrales
et dans les dérivées : on peut concevoir que cela a été fait pour
pouvoir écrire les formules de Green. Cela devrait être dit
explicitement.

-\qquad Il y a une inégalité de traitement des noms de variables :
ce sont des variables (informatiques) pour les dérivées et les
intégrales alors que ce sont des constantes dans les opérations
relatives à la transformation à deux échelles (par exemple pour le
remplacement de B(div(.)) ).

Il faut expliquer pourquoi il est utile d'avoir des noms de
variables qui sont des variables ou des constantes suivant les
fonctions. L'utilisation des deux modes d'utilisation conjoint est
assez dangereux, alors il faut bien le justifier.


\subsubsection{Walid, 8/12}
Preuve Maple:

\begin{itemize}
\item Michel asked to delete the second argument of \texttt{Linearity(i,fun,t)} since
 \texttt{fun} is always \texttt{+}. I think it would be many \texttt{+}'s when we consider
 the typing. I keep this function like this.


\item Some properties (rules) of the two scale are stated in
\texttt{twoscale.mpl}, but they are not stated in the paper neither used in the
automatic proof. To be deleted? Alain: If they are correct wrt the two-scale transform in the paper, keep them
and put just in remark in Appendix C.

\item I added the table \texttt{OnBoundary} in \texttt{hypothesis.mpl}. Notations like
 \texttt{VonBoundary}, \texttt{BVonBoundary}... are replaced with \texttt{OnBoundary[v]},
\texttt{OnBoundary[B[v]]}.

Alain: OK. Revised.

 \item \texttt{IntegrationStrategy} and \texttt{LinearityOf[ScalProd]} are put together.
 Maybe we need a separate file for the classical mathematical properties that include
\texttt{IntegrationStrategy} and \texttt{LinearityOf[ScalProd]}?

Alain: Yes. Added to the TODO list.

\item \texttt{u(0),u(1)} are replaced with \texttt{u0,u1}. Moreover, \texttt{BofZero} 
is replaced with \texttt{LinearityOf(B)}, ...
\end{itemize}

\subsubsection{Alain, 8/12}
Révision Section 4, puis preuve Maple après Walid.

\subsubsection{Alain, 9/12}
Fin révision annexe A et fichiers hypothesis.mpl, twoscale.mpl.
Relecture partie 3 après Walid. Nettoyé, acceptable, mais améliorable.
Au début de about.tex, j'ai ajouté tout ce qui reste à faire dans chaque
partie.

On pourra nous critiquer sur les points suivants

- On s'appuie trop sur une seule preuve, celle du gradient, et on donne
l'impression qu'on n'adapte le langage qu'aux besoins de cette preuve-là
(``ad-hoc''). Il faudrait convaincre de la généralité des solutions poposées.

- On n'a pas prouvé que l'implémentation de notre langage de stratégies est conforme à sa
spécification.


\subsubsection{Alain, 21/12}
Version submitted to JSC committed with SVN number 901.

\subsubsection{Walid, 21/12/2010 (\textbf{Error in the paper and its correction} )}
In the paper Section~\ref{symbtrans:inner:sec} it was stated:
\textit{
With this combinator the desired transformation in our example is }

\texttt{TopDown(InnerContext(div(v,Y\_))(GreenRule))}. 

\textit{\noindent Then the transformation that applies the Green rule until no more $v$
is under a $div$ operator is obtained by application of the
\texttt{Normalizer} combinator to the previous transformation.
Step 8 in the Appendix \ref{appendix:gradient:maple:proof} performs
many applications of Green rules by a single call of this strategy, 
whilst avoiding any risk of non-termination usually associated to Green rules.
This example clearly illustrates the strength of the \texttt{InnerContext} combinator.}


A counter example follows. Recall that
\begin{align*}
\texttt{GreenRule1}:\; \int_{\Omega}A\; div(B)\;dx= -\int_{\Omega}\nabla(A).B\; dx+\int_{\partial
 {\Omega}}\cdots
\end{align*}
And let $\gamma=\texttt{InnerContext(div(v,X\_)(GreenRule))}$. The following 
non terminating applications of $\gamma$ to $t$ are possible: 
\begin{align*}
t= \int_{\Omega}\underbrace{div(v)}_{A}\; div(u)\;dx 
     &\longrightarrow_{\gamma}
            - \int_{\Omega}\nabla(div(v)).u\;dx+ \int_{\partial{\Omega}}\underbrace{\cdots}_{0}\\
     &\longrightarrow_{\gamma} \int_{\Omega}\underbrace{div(v)}_{A}\; div(u)\;dx -\int_{\partial{\Omega}}\underbrace{\cdots}_{0}\\
     & \longrightarrow_{\gamma} \; \cdots
\end{align*}

The point is that \texttt{InnerContext} just requires the presence  of a
 pattern and does not say anything about which factor of $t$ has to be matched
 with $A$ and which factor has to be matched with $B$. Since $t$ matches with
 \texttt{GreenRule1} in two ways, the program can choose \emph{indeterminately}
 one of them. Clearly one of the two matchings  leads to a non terminating
 sequence of  transformations as shown above. 
 \textbf{Solution.} The solution consists in using conditional rules to ensure termination, 
 we redefine $\gamma$ a conditional \texttt{GreenRule1}: 

$\gamma:\; (\texttt{GreenRule1,DependsOn(B,v))}$

where \texttt{DependsOn(B,v)} is a boolean statement that is true iff \texttt{B} 
 has \texttt{v} as a subterm at arbitrary depth. Indeed, \texttt{DependsOn}  
  uses the \texttt{InnerContext} combinator, more examples are in \texttt{memsalab/types}.  

Alain : to integrate in the paper after studying matching and types.  

\newpage
\subsubsection{Alain, 24/06/2011}
Fait, AG, juin 2011 :

Corrections faites dans la preuve mathématique du gradient :

Step 5, pour $\Psi _{2}$ : $\partial_{y_i}$ au lieu de $\partial_{y_j}$,
et $\partial_{x_j}$ au lieu de $\partial_{x_i}$, jusqu'à la fin.


Step 7, correction d'une erreur dans l'approximation (\ref{approx:T:2:eq}) de
$T$ : $x_i$ remplacé par $x_j$, dans toute la suite.


Erreur dans la simplification : Le terme contenant
$$\sum_{j=1}^{n}y_j\partial_{x_j}u^{0}$$ 
est devenu 
$$\sum_{j=1}^{n}\int_{\Omega\times Y} y_j
 \partial_{x_j}\partial_{y_i}v_i\;dxdy$$
  alors qu'il devrait être
$$\sum_{j=1}^{n}\int_{\Omega \times Y} y_j 
 (\partial_{x_j}u^{0}) (\partial_{y_i}v_i)\;dxdy $$
où les parenthèses sont indispensables. De même au Step 8.
Redevient correct au Step 9 sans changement, sauf peut-être
des parenthèses manquantes.


Ajout de parenthèses nécessaires dans la formule de Green du Step 8,
et dans le Step 9. Reste un doute sur le dernier term de $\psi$.


Il manque un remplacement de \texttt{partial(u0*y(j),x(j)}
par \texttt{y(j)*partial(u0,x(j)} à la fin du Step 9, qui vient
du fait que  \texttt{y(j)} ne dépend pas de \texttt{x(j)}.


Corrections faites dans gradient.mpl :

\begin{verbatim}
ApproximationB[2](x(i))(y(i)) -> ApproximationB[2](x(j))(y(j))
\end{verbatim}


Remarque : La fin du step 6 est plus distribuée que son correspondant mathématique.
\subsubsection{28/06/2011}
AG : J'ai commencé à réviser la preuve de l'équation de diffusion.
Voici quelques remarques, puis mes principales modifications.

Remarques :

- Ne pas utiliser evala(Expand quand ce n'est pas nécessaire (step 5).

- Il manquait des simplifications de O() dans la preuve Maple de
  l'équation de diffusion, dès le step 3.

Fait dans la preuve de l'équation de diffusion :
 
Dans diffusion\_equation.tex :

  - Ajout de parenthèses nécessaires pour les
    dérivations partielles.

Dans le code Maple :

- Généralisation de 

\begin{verbatim}
OEpsilonSUM := [
  SUM(BigO(I_,Epsilon),J_,D_),
  DelayEval->BigO(FreshIndex(),Epsilon)];
\end{verbatim}

en 

\begin{verbatim}
OEpsilonSUM2 := [
  SUM(E_ + BigO(I_,Epsilon),J_,D_),
  DelayEval -> SUM(E,J,D) + BigO(FreshIndex(),Epsilon)];
\end{verbatim}

dans convergence.mpl, pour simplifier l'étape 3.
 
- Ajout de \verb!T(f), DelayEval -> f0 + BigO(FreshIndex(),Epsilon)]!
  dans lemmas.mpl, pour l'étape 5.

- Equality replaced by a difference in diffusion\_equation.mpl, to get more
  simplifications.

- Left-hand side of Step 2 more simplified, with 2 extra rules.


FAIT : Sortie de la preuve de l'équation de diffusion en Maple.

\subsubsection{29 juin 2011}
Relecture avec M. Lenczner.

FAIT. Terme en 1/Epsilon en step 9 de la preuve du gradient compris, car on
 fait les étapes 8 et 9 en même temps. Explication ajoutée dans l'article. 

FAIT. Revoir la portée des parenthèses pour les dérivées partielles : minimale.

FAIT. Réponse pour intégrale de Stieljes. Explication ajoutée sur le ds dans la
règle de Green dans la fin du running example. ``The Green rule extends
integration by parts to multidimensional domains'', ``$x \mapsto ds(x)$ is the measure
associated to the boundary of $\Omega$''.
FAIT. Step 6, $a$ ne peut pas être mis dans la fonction de test, car n'a pas les
conditions de régularité. Ici $a$ ne dépend pas de epsilon. Il faut un lemme
pour le produit par une constante : Si $u$ converge faiblement vers $u0$ et $a$
independent of $\epsilon$ then $a u$ converge faiblement vers $a u0$.
$T(a) = a + \ldots$ remplacé par $T(a) = a^0$.

FAIT. Révision de la partie 5.1. Ajout d'une perspective en conclusion.

\subsubsection{4 juillet}
WB : Déplacement du calcul de convergence dans la partie 5. Rédaction de l'ajout
des types et de la modularité dans la conclusion. Ajout citation EuroSIME'11
et CFM'11. Minimal scope assumed for partial derivative.


AG : Fin de la preuve D. k au lieu de j, etc. 


AG: Création du zip de distribution de symbtrans, à l'aide de
/software/memsalab/src/symbtrans/build.xml.

En raison de difficultés techniques pour écrire build.xml (qui ne supporte
ni les chemins relatifs ascendants, ni les chemins absolus), la bibliothèque
symbtrans et les exemples sont déplacés dans des sous-dossiers
de symbtrans, /lib et /examples respectivement. Le chemin vers la librairie
dans les exemples est adapté automatiquement après cette copie.  

\subsubsection{6 juillet}
AG : Dans l'exemple 2, suppression des notations $\mathcal{F}_0$ et  $\mathcal{F}_2$
qui n'ont pas été définies avant. Remplacement par des phrases.

AG : dans rhomaple.tex, ajout de précisions et corrections d'erreurs. Les
précisions sont : Justification de l'absence de levée d'exception par les
``traversal transformations''. Valeur minimale de $n$ précisée dans les
définitions. Les corrections sont : TopDown d'applique aussi aux constantes,
et retourne la transformation du terme entier s'il est différent
Illustration dans la procédure test3() de regtest.mpl.


L'implantation actuelle de TopDown peut échouer sur une règle
conditionnelle.
 
\subsubsection{08/07/2011}
Réunion au LIFC. 


AG : Changement de titre. Dans l'introduction, reformulation de ``Our multiscale
method tries to formalize are based on quasi-systematic derivations of
equalities. The classical way to automate these derivations is to consider
mathematical expressions as symbolic and to give a computational meaning to
mathematical equations. The idea is to orient the equality'', à relire.
 

ML : 2 jours de modifications, puis relecture finale. 


WB : Trois jours de modifications.


AG : Relecture de validation avant mercredi 13, si les modifications sont
terminées avant. 

Inutile de signaler notre retard de soumission aux éditeurs de la revue.
 
\subsection{Related work}
Download and read the papers mentioned in biblioJSC.bib. See also some
PDFs at https://lxsd.femto-st.fr/user/agiorgetti/afmalab/.

Alain : \cite{BKK+99} aborde la question de la r\'e\'ecriture et des strat\'egies
comme nous voulons le faire pour Maple. Il montre les probl\`emes et les r\'esout.
Notre article doit donc le citer, \^etre tr\`es modeste sur l'aspect fondamental de
notre contribution et mettre l'accent sur l'adaptation à Maple, sur l'int\'er\^et
relatif en pratique de telle et telle strat\'egie, \`a travers l'exemple de la
preuve du gradient. Il faut s'inspirer au maximum de ce travail (concepts,
vocabulaire ("primal strategy"), et notation) puis montrer o\`u sont les
diff\'erences. Tu peux m'envoyer cette liste de diff\'erences pour qu'on en discute.


[WB]List of the main concepts and terminology used in \cite{BKK+99}:
\begin{itemize}
\item Elementary strategies, we do not need this, because they are just used to
  formulate the matching algorithm in rule-based way.
\item Primal strategies.
\item Defined strategies.
\item Search strategies.
\item A hierarchy of strategies.
\item Strategy constructor(s).
\item Rewrite system.
\item Rewrite at the top. I prefer head or root rewriting.
\item $\cdots$
\end{itemize}

[Alain: d'accord pour le vocabulaire. Il faut maintenant voir si notre langage
est aussi riche et sinon expliquer pourquoi. ]

Voici qq remarques suite \`a un survol de cet article :

- La fonction qu'on associe \`a une r\`egle de r\'e\'ecriture (ou plus g\'en\'eralement \`a
une strat\'egie) peut \^etre totale ou partielle, typ\'ee ou non.

- Il y a plusieurs mani\`eres de formaliser une fonction partielle. On peut
d'abord se ramener \`a une fonction totale. L'introduction de [BKK+99] sugg\`ere de
le faire en ajoutant une constante pour l'\'echec. Pour une r\`egle de r\'e\'ecriture,
la partie 3.1 de [BKK+99] sugg\`ere de retourner l'ensemble vide, \`a condition que
la fonction ne soit pas typ\'ee (ou, plus g\'en\'eralement, que le typage ne distingue
pas un terme et un ensemble de termes (c'est le cas dans MAUDE, par exemple)).
Nous envisageons plut\^ot d'utiliser un m\'ecanisme d'exceptions, de plus haut
niveau, donc plus l\'eger \`a formaliser.

L'inconv\'enient des exceptions est qu'elles font quitter tout le processus de
transformation. Il faut montrer comment les contr\^oler dans ce processus.

\noindent \textbf{To be clarified}
\begin{enumerate}
\item Either to use names for the abstract  or the effective (functional)  rules (user?).

Alain: I am not sure I understand where is the problem, but I expect
rules/transformations/strategies to be Maple object (pairs, functions, etc) and
thus assignable to a Maple variable with the Maple syntax. Then the question is:
How to access all the previously assigned variables in a Maple program, for
instance to search whether a rule exists?

\item Emphasizing on our functional semantics, its originality, who (which community) cares about it?

Alain : Our functional semantics is not that original, because something similar
has already been done for ELAN~\cite{BKK+99}. But we adapt the ideas of
\cite{BKK+99} to Maple and intensively use the fact that this host language
is functional.

\item Is there a correspondence between the order of (HO) transformations and
that of the (HO) functions?

Alain: See~\cite{BKK+99} or an answer. Where is the problem?

\item Mentioning the type/order of transformations?

Alain: yes, but without emphasizing, just to help organizing the paper
structure. See Section 6 in \cite{BKK+99}.

\item \texttt{Pfun} semantics of transformations (structure of category).

Alain : it is too soon to present this but I keep it in mind when revising the
paper and I will see whether I add a few words about this. Don't focus on this.
Just address me questions that you suspect to have an answer in the theory
of categories.

\item Add a table summarizing rules constructors.

Alain : or a grammar?
\end{enumerate}




\subsubsection{Inner contextual rewriting}
%\noindent \textbf{Inner contextual rewriting}\\
Consider for instance the term
\begin{align*}
 t =&\underbrace{\int_{\Omega  } v \;div_x(u^0) \;dx}_{t_1} 
    %+\int_{\omega \times Y}div_y(\tilde{u}^1)v\;dx 
    +\underbrace{\int_{\Omega }  u^{1}\; div_x(v)\;dx}_{t_2} 
\end{align*}
and the Green rule %\cite{?}
\begin{align*}
\int_{\Omega} A \; div_{x}(B)\;dx= 
    \int_{\partial{\Omega}}  A \;(B.n_{\Omega})\; ds(x) - \int_{\Omega} \nabla_x(A).B \;dx
\end{align*}

where $n_{\Omega}$ denotes the unit outward normal vector to the boundary $\partial(\Omega)$
of $\Omega$.
A computation goal is that the term $v$
 (also called the \emph{test function}, see Section \ref{prelim:sec})
is no longer under a $div$ operator. Thus the right strategy is to apply the
Green rule to the second subterm $t_2$ of $t$, but not to its first subterm
$t_1$. The strategy

\texttt{TopDown(Transform(GreenRule))($t$)}

\noindent is not satisfactory because it applies 
% Notice that if we apply Green rule in a top down way to \texttt{t} by means of
%   then this will apply 
the rule to both $t_1$ and $t_2$. 
To solve this kind of problems we provide
% The solution we suggest consists in providing  
a transformation combinator \texttt{InnerContext(patt)} such that
\texttt{InnerContext(patt)(s)(expr)} 
applies the transformation \texttt{s} to the expression \texttt{expr} 
% at the top 
if and only if \texttt{expr} has a subterm (at some arbitrary depth) 
which matches with the pattern \texttt{patt}. Otherwise it returns the
exception \texttt{"Fail"}.
\begin{displaymath}
 \begin{array}{|l l|}
\hline
  \texttt{InnerContext(patt)(s)(expr)}=_{\textit{def}} & \texttt{if } \exists \texttt{t' subterm of expr } s.t \;\; 
 \match{\texttt{patt}}{\texttt{t'}}   \\ &  \texttt{then  s(expr);} \\
                                        & \texttt{else} \;\; \texttt{Fail();} \\
\hline
\end{array}
\end{displaymath}
With this combinator the desired transformation in our example is 

\texttt{TopDown(InnerContext(div(v,Y\_))(GreenRule))}. 

\noindent Then the transformation that applies the Green rule until  $v$
is no longer under a $div$ operator is obtained by application of the
\texttt{Normalizer} combinator to the previous transformation.
Step 8 in the Appendix \ref{appendix:gradient:maple:proof} performs
many applications of Green rules by a single call of this strategy, 
whilst avoiding any risk of non-termination usually associated to Green rules.
This example clearly illustrates the strength of the \texttt{InnerContext} combinator.

\subsection{Deeply Modified Section}
\subsubsection{Traversal transformations}  
This section introduces transformations called \emph{traversal} or \emph{term}
transformations. These transformations explore the structure of the term
  they are applied on. We provide three traversal transformation
 constructors, namely \texttt{All}, \texttt{TopDown} and \texttt{BottomUp}.
 These three transformations never fail. After a traversal  the
 \texttt{IdentityAsFail} combinator can be invoked to consider
 as a failure that the traversal has left the term unchanged.
  
The transformation \texttt{All(s)} applies the transformation \texttt{s} to all
the immediate subterms of any term \texttt{t}. It is defined by
\begin{displaymath}
\begin{array}{|c l|}
\hline
\texttt{All(s)(t)} =_{\textit{def}} 
 & \texttt{if t=f(t$_1$,$\cdots$,t$_n$) then}\\
 & \hspace{0.4cm}
    \texttt{f(FailAsIdentity(s)(t$_1$),$\cdots$,FailAsIdentity(s)(t$_n$));}\\ 
 & \texttt{else         // t is a constant or a variable} \\
 & \hspace{0.4cm} \texttt{t;} \\
 & \texttt{fi;} \\
 \hline
\end{array}
\end{displaymath}
for $n \geq 1$.

\begin{example}
Consider again the rewrite rule \texttt{IntegralLinearity} of
the example \ref{top:exmp}, encoding the linearity of the integral, and let
$t=\int v(x)+w(x)\;dx$. Notice that the statement 

\texttt{Transform(IntegralLinearity)($t$+2)} 

\noindent raises the exception \texttt{"Fail"} because the rewrite rule cannot
be applied at the top of the expression \texttt{$t$+2}. A solution is to
replace it by the statement

\texttt{All(Transform(IntegralLinearity))($t$+2)} 

\noindent which produces
$\int v(x)\;dx +\int w(x)\;dx + 2$ since the expression
\texttt{$t$+2} is viewed as the term $+(t,2)$.
\end{example}

The transformation \texttt{TopDown(s)} applies the transformation \texttt{s}
to all the subterms of any term \texttt{t}, at any depth, by starting with the
 closest subterms to the root of \texttt{t}:

\begin{displaymath}
\begin{array}{|c l|}
\hline
 \texttt{TopDown(s)(t)} =_{\textit{def}} 
  & \texttt{try }\\ 
  & \hspace{0.4cm} \texttt{u := s(t);}\\
  & \texttt{catch "Fail":} \\
  & \hspace{0.4cm} \texttt{if t = f(t$_1$,...,t$_n$) then}\\
  & \hspace{0.8cm} \texttt{u := f(TopDown(s)(t$_1$), ...,
  TopDown(s)(t$_n$))}\\ & \hspace{0.4cm} \texttt{else         // t is a constant or a variable}
  \\ 
  & \hspace{0.8cm} \texttt{u := t;}\\
  &  \hspace{0.4cm} \texttt{fi;}\\
  & \texttt{end try;} \\
  & \texttt{return(u);}\\
\hline
\end{array}
\end{displaymath}
for $n \geq 1$.




\begin{example}
Let   $t=\int v(x)+w(x) \; dx$,  then 
 
\texttt{TopDown(Transform(IntegralLinearity))($t$*$t$+2)} 

\noindent gives the expression
$(\int v(x) \; dx + \int w(x) \;
dx)*  ( \int v(x) \; dx + \int w(x) \; dx) + 2$, 
since the expression \texttt{$t$*$t$+2} is viewed as the
term $+(*(t,t),2)$.
\end{example}

The transformation \texttt{BottomUp(s)} works as the 
transformation \texttt{TopDown(s)}, but in the opposite direction, i.e. it
applies first the transformation \texttt{s} to the most distant subterms from the
root:
\begin{displaymath}
\begin{array}{|c l|}
\hline
\texttt{BottomUp(s)(t)} =_{\textit{def}}   &\texttt{if ExistChild(s,t) then} \\
   &\hspace{0.4cm} \texttt{All(BottomUp(s))(t);} \\
  & \texttt{else}\\
  & \hspace{0.4cm} \texttt{FailAsIdentity(s)(t);}\\
\hline  
\end{array}
\end{displaymath}
where \texttt{ExistChild(s,t)} returns true iff \texttt{t} has a proper
subterm -- i.e. distinct from \texttt{t} -- on which \texttt{s} can be applied.

The transformation \texttt{BottomUp(s)} is not used in the proof reproduced in
Appendix~\ref{appendix:gradient:maple:proof}.  However it is very common in
practice;  most  programming languages evaluate the
 arguments of a function before evaluating the function itself.
Moreover, including it in \ST puts its strategy language at the same level of
expressiveness as the \textsc{Tom}
 strategy language, see \cite{BBK_Tom07}, in terms
  of transformation constructors.


Finally, we mention that, for practical reason, \ST is implemented so that 
 one uses the function \texttt{Transform(r)}  only 
 when the  rule \texttt{r} has to be applied at the top, otherwise, if 
\texttt{r} is applied according to a  strategy then there is no need to write 
\texttt{Transform}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "0"
%%% End:


==> contextual.tex <==
\subsection{Contextual transformations} 
When dealing with the proof of the derivative weak convergence property (Appendices
\ref{appendix:gradient:math:proof} and \ref{appendix:gradient:maple:proof}), we
have faced situations where rule application should depend on the
\emph{context} of a subterm.  We distinguish two notions of context: \emph{(i)} the
\emph{inner} context -- where some conditions are imposed on some descendant of
the subterm --  and  \emph{(ii)}  the \emph{outer} context -- where conditions
are imposed on some ancestor of the subterm. We define one
contextual combinator for each case.
%  The advantage of the contextual combinators is a
% practical one: we do not need to write as many rewrite rules as the number of different contexts.

\subsubsection{Inner contextual rewriting}
\label{symbtrans:inner:sec}
Suppose you want to apply the Green rule, i.e. Eq. (\ref{Green Formula}), to
the term
\begin{align*}
 t =&\underbrace{\int_{\Omega  } v \;\partial_{x_i}u^0 \;dx}_{t_1} 
    +\underbrace{\int_{\Omega }  u^{1}\; \partial_{x_i}v \;dx}_{t_2} 
\end{align*}

so  that the term $v$
 (also called the \emph{test function}, see Section \ref{prelim:sec})
is no longer under the differentiation operator $\partial$. The right strategy
is to apply the Green rule to the second subterm $t_2$ of $t$, but not to its
first subterm $t_1$. The strategy

\texttt{\STTop(Transform(GreenRule))($t$)}

\noindent is not satisfactory because it applies 
% Notice that if we apply Green rule in a top down way to \texttt{t} by means of
%   then this will apply 
the rule to both $t_1$ and $t_2$. 
To solve this kind of problems we provide
% The solution we suggest consists in providing  
the transformation combinator \texttt{InnerContext} such that
\texttt{Inner\-Context}$(p)(s)(t)$ applies the transformation $s$ to the expression $t$ 
if and only if $t$ has a subterm (at some arbitrary depth) 
which matches with the pattern $p$. Otherwise it raises the
exception \texttt{"Fail"}.
\begin{displaymath}
 \begin{array}{|l l|}
\hline
  \texttt{InnerContext}(p)(s)(t) =_{\textit{def}} 
   & \texttt{if } \exists \texttt{t' subterm of t } s.t \;\; \match{\texttt{p}}{\texttt{t'}}
      \texttt{ then}  \\ 
  & \hspace{0.6cm} \texttt{s(t);} \\ 
  & \texttt{else} \;\; \\
  & \hspace{0.6cm}  \texttt{Fail();} \\
  & \texttt{fi;} \\
\hline
\end{array}
\end{displaymath}
With this combinator the desired transformation in our example is 

\texttt{\STTop(InnerContext(partial(v,Y\_))(GreenRule))}. 

\noindent Then the transformation that applies the Green rule until  $v$
is no longer under the $\partial$ operator is obtained by application of the
\texttt{STNormalizer} combinator to the previous transformation. Notice
that such transformation  may not terminate, e.g. when it is applied
to the term $\int_{\Omega}\partial_{x_i}u\, \partial_{x_i}v \;dx$. 
Notice that even the refinement of \texttt{InnerContext} by a conditional
rule - as in Step 8 in the Appendix \ref{appendix:gradient:maple:proof} -
 does not ensure termination in the general case.
%% Step 8 in the Appendix \ref{appendix:gradient:maple:proof} performs
%% many applications of Green rules by a single call of this strategy, 
%% whilst avoiding any risk of non-termination usually associated to Green rules.
%% This example clearly illustrates the strength of the \texttt{InnerContext} combinator.


\subsubsection{Outer contextual rewriting}
For an example of rewriting under an outer context, consider the term
\begin{align*}
  t = -\int_{\Omega}u \underbrace{B(\partial_{x_i} v)}_{t_1} dx -
       \int_{\Omega} \frac{1}{\varepsilon}u \underbrace{B(\partial_{y_i}v)}_{t_2} dx +
       O(\varepsilon)
\end{align*}
and the problem of approximating $t_1$ and $t_2$ so as to get a first-order
approximation in $\varepsilon$ of $t$. The rewrite rule \texttt{ApproximationB1}:
$\rrule{B(w\_)}{T^*w+O(\varepsilon)}$ is convenient for $t_1$ but not for $t_2$,
due to the multiplicative factor $\frac{1}{\varepsilon}$. For $t_2$ the
 rule \texttt{ApproximationB2}: $\rrule{B(w\_)}{T^*(w)+
\varepsilon \sum_{i=1}^{n} y_i \, T^*(\partial_{x_i} w) +\varepsilon O(\varepsilon)}$ is required. Notice
that both rules have the same left-hand side. Therefore the application of one of
them to $t$ in a top-down way would give an unwanted result.  


We propose a solution based on 
%\emph{higher-order rewriting}, i.e.
%Confusion with rewriting calculus: there, Hi.Order means arbitrary rho-terms 
 the ability to
apply rewrite rules to rules themselves in order to produce new rules. In the
present example, the 
%(second-order) 
rule

\texttt{multContext := }$\rrule{X\_}{\frac{1}{\varepsilon}XY\_}$ 

\noindent could transform the 
%(first-order)
 rule \texttt{ApproximationB2}
into the  %(first-order)
 rule 
\begin{align*}
\rrule{\frac{1}{\varepsilon} B(w\_) Y\_}{\frac{1}{\varepsilon} \left(T^*(w)+
\varepsilon \sum_{i=1}^{n}y_i \, T^*(\partial_{x_i} w) +\varepsilon O(\varepsilon)\right) Y\_}
\end{align*}
that takes into account the useful part of the outer context, i.e. the
multiplicative factor $\frac{1}{\varepsilon}$.


We define the transformation constructor \texttt{OuterContext} as follows. Let
$r$ be a rewrite rule and $c$ be a \emph{context} rule designed to add a
context to $r$. The rule transformation
\texttt{OuterContext}$(r)(c)$ applies $c$ to the left- and
right-hand sides of the rewrite rule $r$ and returns the contextualization of
$r$ by $c$. In the example the contextualized rule

\texttt{r\_epsilon := OuterContext(ApproximationB2)(multContext)}

\noindent provides a solution to the problem. After
Maple$^{\mathsf{TM}}$ simplifications, its value is 
\begin{align*}
\rrule{\frac{1}{\varepsilon} B(w\_) Y\_}{(\frac{1}{\varepsilon}T^*(w)+ 
\sum_{i=1}^{n}y_i\, T^*(\partial_{x_i} w) + O(\varepsilon)) Y}.
\end{align*}
Notice that the presence of the variable \texttt{Y\_}  in the right-hand side of
the rule \texttt{multContext} is necessary. Otherwise the resulting rule
\texttt{r\_epsilon} would not be applicable if the term
contains other factors than $\frac{1}{\varepsilon}$ and $B(\ldots)$. 
Finally, the desired transformation is

\begin{verbatim}
 Comp([
  Outermost(Transform(r_epsilon)),
  Innermost(Transform(ApproximationB1))]).
\end{verbatim}


==> correspondance.tex <==

Table~\ref{math:maple:notation:table} establishes the correspondence between the
notations used in the mathematical proofs and in the formal ones. Table
\ref{math:maple:rule:table} associates rewrite rules to mathematical lemmas and
equations.

\begin{table}[htb]
\begin{displaymath}
 \begin{array}{|c| l|}
\hline
\textrm{Mathematical notations} &\texttt{Formal notations}\\
\hline
 T^{\star}  & \texttt{TS} \\
  \Omega    & \texttt{Omega}\\
   \widetilde{\Omega}    & \texttt{TSTM(Omega)}\\
  Y   &  \texttt{TSTm(Omega)}\\
 \partial_x v & \texttt{partial(v,x)}\\
(n_{\Omega}) & \texttt{n(Omega)}\\
O(\varepsilon) & \texttt{BigO(FreshIndex(),Epsilon)}\\
\partial \Omega & \texttt{partialBound(Omega,x)}\\
\sum_{i\in I}f & \texttt{SUM(f,i,I)} \\
\int_{\Omega}f\, dx & \texttt{Integral(Omega,f,x)} \\
\int_{\Omega \times Y} f \, dxdy & \texttt{Integral([Omega,Y],f,[x,y])} \\
A\times B \text{ (i.e. Cartesian product)} & [A,B] \text{ (i.e. Maple list)}\\
a^0, u^0, u^1, \ldots & \texttt{a0, u0, u1}, \ldots\\
\hline
\end{array}
\end{displaymath}
\caption{Correspondence between mathematical and formal
notations\label{math:maple:notation:table}}
\end{table} 



\begin{table}[htb]
\begin{center} 
\begin{tabular}{|c| l|}
\hline
Mathematical properties &\texttt{Rewriting rule names}\\
\hline
Lemma 8  & \texttt{TwoScaleAdjointInv} \\
Lemma 9  & \texttt{ApproximationTS[1]} \\
 \textrm{a function vanishing on a boundary}     & \texttt{IntegralOnBoundary} \\
Eq. \ref{B:derivative}   & \texttt{PartialOfB} \\  
Eq. \ref{B:approximation:1} & \texttt{ApproximationB[1]} \\
Eq. \ref{B:approximation:2} & \texttt{ApproximationB[2]} \\
Eq. \ref{T:adjoint:eq}& \texttt{TwoScaleAdjoint} \\
Eq. \ref{approx:T:1:eq}  & \texttt{ApproximationT[1]} \\
Eq. (\ref{approx:T:2:eq}) & \texttt{ApproximationT[2]} \\
$2^{\textrm{nd}}$ Eq. \textrm{ of  assumption } (\ref{model:diffusion:assumption})
  &\texttt{ApproximationT[3]} \\
Eq. (\ref{gradient:prop:limit}) & \texttt{GradientApprox} \\ 
Eq. (\ref{Green Formula}) & \texttt{GreenRule}\\
\hline
\end{tabular}
\caption{Correspondence between mathematical properties and rewriting
rules\label{math:maple:rule:table}}
\end{center}
\end{table} 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 



==> gradient-input.tex <==
# Initial term
LHSterm := Integral(
 {TSTM(Omega),Y},
 T(gradient(u,x))*v,
 {x,y});

# Step 1
LHSterm := Transform("TwoScaleAdjointInv",LHSterm);

# Step 2
LHSterm := Transform(TopDown("ApproximationTS"),LHSterm);
LHSterm := evala(Expand(LHSterm));
LHSterm := Transform("Integral_sum",LHSterm);
LHSterm := Transform(TopDown("OEpsilonIntegral"),LHSterm);
LHSterm := Transform(TopDown("GreenRule"), LHSterm);

DeclareRule(
 "Boundary1",
 Integral({gradient(A_)},F_*bar(v),X_),
 0):
LHSterm:=Transform(TopDown("Boundary1"),LHSterm);
LHSterm:= Transform(TopDown("BarBasicPropertyDiv"),LHSterm);
LHSterm:=evala(Expand(LHSterm));
LHSterm:=Transform(TopDown("Integral_sum"), LHSterm);

#Step 5:
fprintf(traceFile,"----- LHSTERM 5 ---------\n");
subterm1:=bar(div(v, {x}));
LHSterm:=sub(subterm1,Transform("ApproximationTSInv1",subterm1),LHSterm);
subterm2:=bar(div(v, {y}));
LHSterm:=sub(subterm2,Transform("ApproximationTSInv2",subterm2),LHSterm);
LHSterm := evala(Expand(LHSterm));
LHSterm := sub(A_*(1/Epsilon)*TS(V_),A*TS(1/Epsilon*V),LHSterm);
LHSterm := evala(Expand(LHSterm));
LHSterm:=Transform(TopDown("Integral_sum"),LHSterm);
LHSterm:=Transform(TopDown("Integral_sum"),LHSterm);
LHSterm := Transform(TopDown("OEpsilonIntegral"),LHSterm);

#Step 6
LHSterm:=Transform(TopDown("TwoScaleAdjoint"),LHSterm);

#Step 7
LHSterm:=sub( div(A_,B_)*T(u) , 
            div(A,B)*( u({0})+BigO(FreshIndex(),Epsilon)),
            LHSterm);
LHSterm := sub( T(u), 
                u({0}) + Epsilon*tilde(u({1})) +  Epsilon*BigO(FreshIndex(),Epsilon),
                LHSterm);
LHSterm:= evala(Expand(LHSterm));
LHSterm:=Transform(NF(TopDown("Integral_sum")),LHSterm);
LHSterm:= Transform(TopDown("EpsilonConst"),LHSterm);
LHSterm:= Transform(TopDown("OEpsilonIntegral"),LHSterm);
LHSterm:= Transform(TopDown("OEpsilonConst"),LHSterm);
LHSterm:=sub(Integral(Var_, (div(v, {y})*u({0}))/Epsilon,V_),0,LHSterm);
fprintf(traceFile," %a \n",LHSterm):

#Step 8
LHSterm:=Transform(TopDown("GreenRuleDiv"),LHSterm);
LHSterm:=Transform(TopDown("GreenRulePartial"),LHSterm);

DeclareRule(
 "Boundary2",
 Integral({partial(A_)},F_*bar(v),X_),
 0):
LHSterm:=applyrule(Integral(set(partial(E_::algebraic)),V_::algebraic,X_::algebraic)=0,LHSterm);
LHSterm:=sub(Integral(Omega_, X_ * div(v,D_), A_),Transform("GreenRuleDiv",Integral(Omega, X*div(v,D), A)),LHSterm);
 LHSterm:=applyrule(Integral(set(partial(X::anything)),C::anything,Y::anything)= 0,LHSterm);

#Step 9
LHSterm:=sub( tilde(u({1})), u({1})+y*div(u({0}),x),LHSterm);
LHSterm:= sub( div(y*u({0}), x) ,y*div(u({0}), x),LHSterm);
LHSterm:= evala(Expand(LHSterm));
#Linearity of div
DeclareRule("Dist_div_sum",div(A_+B_,X_),div(A,X) + div(B,X)):

LHSterm:=Transform(TopDown("Dist_div_sum"),LHSterm);
LHSterm:=evala(Expand(LHSterm));
LHSterm:=Transform(TopDown("Integral_sum"),LHSterm);

#RHSterm
RHSterm:=Integral(
   {Y,TSTM(set(Omega))},
   v*div(u({0}),{x}) + v*div(u({1}),{y}),
   {x,y})+BigO(FreshIndex(),Epsilon);

RHSterm:=Transform(TopDown("Integral_sum"),RHSterm);

Result:=Transform(NF(TopDown("OEpsilonConst")),LHSterm-RHSterm);


==> gradient-output.tex <==
------ Reduction Of Left Hand Side Term--------
------ STEP 1 --------
 Integral({Y, TSTM(Omega)},T(gradient(u,x))*v,{x, y})
=
 Integral(Omega,TS(v)*gradient(u,x),{x})
----- STEP 2 ---------
=
 Integral(Omega,(bar(v)+BigO(1,Epsilon))*gradient(u,x),set(x))
=
 Integral(Omega,gradient(u,x)*bar(v)+gradient(u,x)*BigO(1,Epsilon),set(x))
=
 Integral(Omega,gradient(u,x)*bar(v),set(x))+Integral(Omega,gradient(u,x)*BigO(1,Epsilon),set(x))
=
 Integral(Omega,gradient(u,x)*bar(v),set(x))+BigO(5,Epsilon)
------- STEP 3 -------
=
 Integral({gradient(Omega)},u*bar(v)*Eta(x),{x})-Integral({Omega},u*div(bar(v),{x}),{x})+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*div(bar(v),set(x)),set(x))+BigO(5,Epsilon)
----- LHSTERM 4 ---------
=
 -Integral(set(Omega),u*(bar(div(v,set(x)))+1/Epsilon*bar(div(v,{y}))),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*bar(div(v,set(x)))+u/Epsilon*bar(div(v,{y})),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*bar(div(v,set(x))),set(x))-Integral(set(Omega),u/Epsilon*bar(div(v,{y})),set(x))+BigO(5,Epsilon)
----- LHSTERM 5 ---------
=
 -Integral(set(Omega),u*(TS(div(v,{x}))+BigO(3,Epsilon)),set(x))-Integral(set(Omega),u/Epsilon*bar(div(v,set(y))),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*(TS(div(v,set(x)))+BigO(3,Epsilon)),set(x))-Integral(set(Omega),u/Epsilon*(TS(div(v,{y})+Epsilon*y*partial(div(v,{y}),x))+Epsilon*BigO(4,Epsilon)),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x)))+u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u/Epsilon*TS(div(v,{y})+Epsilon*y*partial(div(v,{y}),x))+u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x)))+u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*(div(v,{y})+Epsilon*y*partial(div(v,{y}),x)))+u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x)))+u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*div(v,{y})+y*partial(div(v,{y}),x))+u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon)
=
 -Integral(set(Omega),u*TS(div(v,set(x))),set(x))-Integral(set(Omega),u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*div(v,{y})+y*partial(div(v,{y}),x)),set(x))-Integral(set(Omega),u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon) 
=
 -Integral(set(Omega),u*TS(div(v,set(x))),set(x))-Integral(set(Omega),u*BigO(3,Epsilon),set(x))-Integral(set(Omega),u*TS(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x)),set(x))-Integral(set(Omega),u*BigO(4,Epsilon),set(x))+BigO(5,Epsilon) 
=
 -Integral(set(Omega),u*TS(div(v,set(x))),set(x))-BigO(5,Epsilon)-Integral(set(Omega),u*TS(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x)),set(x))
----- LHSTERM 6 ---------
=
 -Integral({Y, TSTM(set(Omega))},div(v,set(x))*T(u),{x, y})-BigO(5,Epsilon)-Integral({Y, TSTM(set(Omega))},(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x))*T(u),{x, y})
------ LHSTERM 7 --------
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*(u({0})+BigO(9,Epsilon)),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x))*T(u),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*(u(set(0))+BigO(9,Epsilon)),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),(1/Epsilon*div(v,set(y))+y*partial(div(v,set(y)),x))*(u({0})+Epsilon*tilde(u({1}))+Epsilon*BigO(10,Epsilon)),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0))+div(v,set(x))*BigO(9,Epsilon),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u({0})+div(v,set(y))*tilde(u({1}))+div(v,set(y))*BigO(10,Epsilon)+y*partial(div(v,set(y)),x)*u({0})+y*partial(div(v,set(y)),x)*Epsilon*tilde(u({1}))+y*partial(div(v,set(y)),x)*Epsilon*BigO(10,Epsilon),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*BigO(9,Epsilon),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*BigO(10,Epsilon),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*Epsilon*BigO(10,Epsilon),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*Epsilon*tilde(u(set(1))),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*BigO(9,Epsilon),set(x,y))-BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*BigO(10,Epsilon),set(x,y))-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))-2*Integral(set(Y,TSTM(set(Omega))),7*BigO(8,Epsilon),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))-5*BigO(5,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))+BigO(6,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),1/Epsilon*div(v,set(y))*u(set(0)),set(x,y))
=
 -Integral(set(Y,TSTM(set(Omega))),div(v,set(x))*u(set(0)),set(x,y))+BigO(6,Epsilon)-Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*tilde(u(set(1))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y)) 
------ LHSTERM 8  --------
=
 -Integral({partial(set(Y,TSTM(set(Omega))))},v*u(set(0))*Eta(set(x)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)-Integral({partial(set(Y,TSTM(set(Omega))))},v*tilde(u(set(1)))*Eta(set(y)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),y*partial(div(v,set(y)),x)*u(set(0)),set(x,y)) 
=
 -Integral(set(partial(set(Y,TSTM(set(Omega))))),v*u(set(0))*Eta(set(x)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)-Integral(set(partial(set(Y,TSTM(set(Omega))))),v*tilde(u(set(1)))*Eta(set(y)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))-Integral({partial(set(Y,TSTM(set(Omega))))},div(v,set(y))*y*u(set(0))*Eta(x),set(x,y))+Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*div(y*u(set(0)),x),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))+Integral(set(Y,TSTM(set(Omega))),div(v,set(y))*div(y*u(set(0)),x),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))+Integral({partial(set(Y,TSTM(set(Omega))))},v*div(y*u(set(0)),x)*Eta(set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(div(y*u(set(0)),x),set(y)),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(tilde(u(set(1))),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(div(y*u(set(0)),x),set(y)),set(x,y)) 
------ LHSTERM 9  --------
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u({1})+y*div(u({0}),x),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(div(y*u(set(0)),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(1))+y*div(u(set(0)),x),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u({0}),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(1))+y*div(u(set(0)),x),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u({0}),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*(div(y*div(u(set(0)),x),set(y))+div(u(set(1)),set(y))),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u(set(0)),x),set(y)),set(x,y)) 
=
Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u(set(0)),x),set(y))+v*div(u(set(1)),set(y)),set(x,y))-Integral(set(Y,TSTM(set(Omega))),v*div(y*div(u(set(0)),x),set(y)),set(x,y)) 
=
 Integral(set(Y,TSTM(set(Omega))),v*div(u(set(0)),set(x)),set(x,y))+BigO(6,Epsilon)+Integral(set(Y,TSTM(set(Omega))),v*div(u(set(1)),set(y)),set(x,y)) 
------ Reduction Of Right Hand Side Term--------
=
 Integral({Y, TSTM(set(Omega))},v*div(u({0}),{x})+v*div(u({1}),{y}),{x, y})+BigO(11,Epsilon) 
=
 Integral({Y, TSTM(set(Omega))},v*div(u({0}),{x}),{x, y})+Integral({Y, TSTM(set(Omega))},v*div(u({1}),{y}),{x, y})+BigO(11,Epsilon) 
------------------------------ 
------  The  Left and Right Hand Side Terms matches up to:
=
 BigO(6,Epsilon) 


==> multiscale.tex <==
\mycomment{WB}{This section to be deleted}
\begin{itemize}
\item Introduction to the required two-scale transform operators and properties  from Michel notes. 
 \begin{itemize}
 \item Motivations: need for simplified models, approximate model when the number of components is height.
\item Periodic models: homogenization method.
\item Definition of 2-scale transform $T$ and its algebraic properties, adjoint  of $T$.
\item Remaining operators, namely the regularization $\overline{v}$.      
 \end{itemize}

\item Recall how to convert an equational to a rewrite rule. Types and hypothesis
about the operators are not considered, we just focus on the untyped
transformations.
\end{itemize}

\begin{prop}\label{gradient:approx:prop}
$T(\nabla u)$  converges weakly towards $\nabla_x u^0 + \nabla_y u^1$, that is 
\begin{align} \label{Aim:eq}
\underbrace{\int_{\omega \times Y}T(\nabla u).v \; dxdy}_{\Psi}=
 \int_{\omega \times Y}    (\nabla_x u^0 + \nabla_y u^1).v \;\;  dxdy + O(\varepsilon)
\end{align}

\end{prop}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 


==> rule-packages-explanations.tex <==
The proof-independent rewrite rules and transformation terms that correspond to
\emph{two scale transform properties}, \emph{convergence calculus}, \emph{Green
 rules}, and \emph{integral rules}, and the proof-dependent ones that are the
 proof \emph{hypotheses} and \emph{lemmas} are separated in different Maple
 files. All these files are reproduced in Appendix~\ref{appendix:rules}.
% This appendix contains the and they are used by the main proof file given in
% Appendix B.


The collection of mathematical functions and their behavior on the boundary of
the region $\Omega$ is stored in an array named \texttt{OnBoundary}.


An execution of this formal proof with Maple, after loading the \ST package and
all the files reproduced in Appendix~\ref{appendix:rules}, returns the expected
result that the left- and right-hand sides of Equation~(\ref{Expansion of Tu})
are equal modulo some $\OEpsi{\ldots}$.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 

